Tutorials on Testing Neural Networks

Deep learning achieves remarkable performance on pattern recognition, but can be vulnerable to defects of some important properties such as robustness and security. This tutorial is based on a stream of research conducted since the summer of 2018 at a few UK universities, including the University of Liverpool, University of Oxford, Queen's University Belfast, University of Lancaster, University of Loughborough, and University of Exeter. The research aims to adapt software engineering methods, in particular software testing methods, to work with machine learning models. Software testing techniques have been successful in identifying software bugs, and helping software developers in validating the software they design and implement. It is for this reason that a few software testing techniques -- such as the MC/DC coverage metric -- have been mandated in industrial standards for safety critical systems, including the ISO26262 for automotive systems and the RTCA DO-178B/C for avionics systems. However, these techniques cannot be directly applied to machine learning models, because the latter are drastically different from traditional software, and their design follows a completely different development life-cycle. As the outcome of this thread of research, the team has developed a series of methods that adapt the software testing techniques to work with a few classes of machine learning models. The latter notably include convolutional neural networks, recurrent neural networks, and random forest. The tools developed from this research are now collected, and publicly released, in a GitHub repository: \url{https://github.com/TrustAI/DeepConcolic}, with the BSD 3-Clause licence. This tutorial is to go through the major functionalities of the tools with a few running examples, to exhibit how the developed techniques work, what the results are, and how to interpret them.

==> datasets.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Example Datasets}
\label{sec:datasets}

\subsection{Fashion-MNIST}

\input{fm}

\subsection[HAR]{Human Activity Recognition}

\input{har}

% Local variables:
% TeX-master: "slides-intro"
% End:

% LocalWords:  Dataset Triaxial


==> dc-update.tex <==
% -*- coding: utf-8; mode: latex -*-

\begin{frame}[fragile]{\insertsubsection}
  \begin{block}{Updating}<+->
    \begin{itemize}
    \item In the \inlinesh{DeepConcolic} directory retrieved from git at the first session:
\begin{cmds}
git pull
\end{cmds}
      \medskip
    \item In case some files have been modified locally:
\begin{cmds}
git stash && git pull && git stash pop
\end{cmds}
    \end{itemize}
  \end{block}
  \bigskip
  \begin{alertblock}{Activating the Environment}<+->
    \begin{itemize}
    \item[]
% !setup conda conda-activate
\begin{cmds}
conda activate deepconcolic
\end{cmds}
    \end{itemize}
  \end{alertblock}
\end{frame}

% Local variables:
% TeX-master: "slides-all"
% End:


==> deepconcolic-high-level-demo.tex <==
% -*- coding: utf-8; mode: latex -*-

\begin{frame}{\insertsubsection~with \DeepConcolic}
  \begin{block}{Workflow for Live Demos}
  \begin{enumerate}
  \item Using the \dbnabstr companion tool to construct the BN abstraction\par
    \hfill(compute the \(λ_i\)'s and the \(\mathsf{discr}^{♯}_i\)'s)\par
  \item Re-use the BN abstraction with \DeepConcolic for test case generation
  \end{enumerate}
  \end{block}
\end{frame}

\subsection{Relevant Command-line Options for \dbnabstr}

\begin{frame}{\insertsubsection}
  \begin{block}{General}
    \begin{itemize}
    \item \shparambox{--dataset $D$ --model $\mathit{DNN}$ --rng-seed $n$}, (as for \shparambox{deepconcolic.main})
    \item \shparambox{\{create|show\} $\mathit{abstraction\mbox-file}$}
    \end{itemize}
  \end{block}
  \begin{block}{Feature Extraction}
    \begin{itemize}
    \item Layer selection: \shparambox{--layers $\mathit{layer~names}$}
    \item Feature extraction technique: \shparambox{--feature-extraction \{pca, ipca, ica\}}
    \item Number of features to extract for each layer: \shparambox{--num-features $n$}
    \item Training dataset size: \shparambox{--train-size $|\Xtrain|$}
    \end{itemize}
  \end{block}
  \begin{block}{Hidden Feature Discretisation}
    \begin{itemize}
    \item Number of intervals for each extracted feature: \shparambox{--num-intervals $m$}
    \item Discretisation strategy: \shparambox{--discr-strategy \{uniform, quantile\}}
    \item With \shparambox{--extended-discr}, the \(m\) intervals include at least two left- and right-open intervals that are not exercised by \Xtrain
    \end{itemize}
  \end{block}
\end{frame}

\subsection{Relevant Command-line Options for \DeepConcolic}

\begin{frame}[allowframebreaks]{\insertsubsection}
  \begin{block}{General}
    \begin{itemize}
    \item \shparambox{--dataset $D$ --model $\mathit{DNN}$},
    %   (as for \shparambox{deepconcolic.eval\_classifier})
    % \item
      \shparambox{--outputs $\mathit{directory}$},
      \shparambox{--init $|X_0|$}, \shparambox{--max-iterations $N$},
      \shparambox{--save-all-tests}, \shparambox{--rng-seed $n$}
    \end{itemize}
  \end{block}
  \begin{block}{Exploration}
    \begin{itemize}
    \item Norm for Oracle and Search Engine: \shparambox{--norm \{l0,linf\}}
    \item Test Criterion: \shparambox{--criterion \{bfc, bfdc\}}
    \item BN Abstraction: \shparambox{--bn-abstr $\mathit{abstraction\mbox-file}$}
    \end{itemize}
  \end{block}
  \begin{exampleblock}{Examples}
    \begin{itemize}
    \item \(L_0\) exploration for feature coverage: \shparambox{--norm l0 --criterion bfc}
    \item \(L_∞\) exploration via concolic testing for feature coverage: \shparambox{--norm linf --criterion bfc}
    \item \(L_∞\) exploration via concolic testing for feature-dependence coverage: \shparambox{--norm linf --criterion bfdc}
    \end{itemize}
  \end{exampleblock}
  \framebreak
  \begin{block}{Oracle}
    \begin{itemize}
    \item Distance threshold for the oracle: \shparambox{--norm-factor $\dthr$}
    \item[] (defaults to \(\frac 1 4\) for \(L_∞\), \(\frac{|\mbox{input features}|} 4\) for \(L_0\))
    \item Outlier/novelty detection for non-image data: \shparambox{--filters LOF}
    \end{itemize}
  \end{block}
  \begin{block}{Concolic Testing% (\(L_∞\) norm)
    }
    \begin{itemize}
    \item Hard lower-bound for \(\|x - x'\|_∞\): \shparambox{--lb-hard $\dminHard$}
      \hfill(\(\dminHard ∈ [0,1[\))
    \item Noise for the lower-bound of \(\|x - x'\|_∞\): \shparambox{--lb-noise $\dminNoise$}
      \hfill(\(\dminNoise ∈ [0,1-\dminHard[\))
    \item Enforce \(\|x-x'\|_∞ ≥ \dminHard + d'\), with \(d' \sim U(0,\dminNoise)\)
    \end{itemize}
  \end{block}
  % \begin{block}{Gradient Analysis}
  %   \begin{itemize}
  %   \item \shparambox{--mcdc-cond-ratio $r$} consider activations of a ratio $r$ of neurons in condition layers (instead of a single neuron)\hfill (defaults to \(\frac 1 {100}\))
  %   \end{itemize}
  % \end{block}
\end{frame}

\subsection{\DeepConcolic~--- Live Demos with Fashion-MNIST}

\input{dc-update}

\input{fm}

\subsubsection{Creating a BN Abstraction}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  % !deepconcolic dbnc create fashion-mnist medium pca
\begin{cmds}
python3 -m deepconcolic.dbnabstr --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 create outs/fm-medium/bn.pkl --feature-extraction pca --num-features 3 --num-intervals 3 --extended-discr --layers activation activation_1 activation_2 --train-size 10000
\end{cmds}
\begin{textcode}
…
Using extended 3-bin discretizer with uniform strategy for layer activation
Using extended 3-bin discretizer with uniform strategy for layer activation_1
Using extended 3-bin discretizer with uniform strategy for layer activation_2

| Given 10000 classified training sample
| Extracting and discretizing features for layer activation...
| Extracted 3 features
| Discretization of feature 0 involves 3 intervals
| Discretization of feature 1 involves 3 intervals
| Discretization of feature 2 involves 3 intervals
| Discretized 3 features
…
| Captured variance ratio for layer activation is 16.60%
| Captured variance ratio for layer activation_1 is 18.60%
| Captured variance ratio for layer activation_2 is 46.70%
| Created Bayesian Network of 9 nodes and 18 edges.
Dumping abstraction into `outs/fm-medium/bn.pkl'... done
\end{textcode}
\end{frame}

\subsubsection{Inspecting the BN Abstraction}
\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  % !deepconcolic dbnc show fashion-mnist medium pca
\begin{cmds}
python3 -m deepconcolic.dbnabstr --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 show outs/fm-medium/bn.pkl
\end{cmds}
\begin{textcode}
===  Extracted Features and Associated Intervals  ==============================
Layer         Feature    Intervals
------------  ---------  -----------------------------------------
activation    0          (-inf, -66.3), [-66.3, 106), [106, inf)
              1          (-inf, -89.6), [-89.6, 106), [106, inf)
              2          (-inf, -54.5), [-54.5, 123), [123, inf)
activation_1  0          (-inf, -45.4), [-45.4, 47.9), [47.9, inf)
              1          (-inf, -36), [-36, 56.3), [56.3, inf)
              2          (-inf, -41.5), [-41.5, 52.6), [52.6, inf)
activation_2  0          (-inf, -7.57), [-7.57, 9.13), [9.13, inf)
              1          (-inf, -6.01), [-6.01, 10.8), [10.8, inf)
              2          (-inf, -9.9), [-9.9, 10.9), [10.9, inf)
\end{textcode}
\end{frame}

\subsubsection{Feature Coverage with Pixel\-wise Optimisation (\(L_0\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic dbnc fashion-mnist medium bfc l0
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/bfc-l0 --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --bn-abstr outs/fm-medium/bn.pkl --criterion bfc --norm l0 --save-all-tests --init 100 --max-iterations 100
\end{cmds}
\begin{textcode}
…
#0 BFC: 33.33333333%
| Targeting interval (-inf, -66.3) of feature 0 in layer activation (from test 40)
#1 BFC: 81.48148148% with new test case at L0 distance 3: passed
…
| Targeting interval [123, inf) of feature 2 in layer activation (from test 102)
#6 BFC: 100.00000000% with new test case at L0 distance 15: passed
Terminating after 6 iterations: 6 tests generated, 0 of which is adversarial.
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=5cm, trim={0 56px 0 56px}, clip]{%
      res/fm-medium-bfc-l0-ok-montage.png}%
    \includegraphics[width=5cm, trim={0 0 0 112px}, clip]{%
      res/fm-medium-bfc-l0-ok-montage.png}%
  }\par
\end{frame}

\subsubsection{Visualisation of Test Records}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !recviz dbnc fashion-mnist medium bfc l0
\begin{cmds}
pip3 install pyvis
python3 -m deepconcolic.recviz outs/fm-medium/bfc-l0/record-20210407-110118.yml
\end{cmds}
  \medskip
  \centering
  \includegraphics[width=\textwidth]{diagrams/recviz.png}
\end{frame}

\subsubsection{Feature Coverage with Concolic Search Engine (\(L_∞\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic dbnc fashion-mnist medium bfc linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/bfc-linf --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --bn-abstr outs/fm-medium/bn.pkl --criterion bfc --norm linf --save-all-tests --init 100 --max-iterations 10
\end{cmds}
\begin{textcode}
…
Initializing with 100 randomly selected test cases that are correctly classified.
#0 BFC: 33.33333333%
| Targeting interval (-inf, -66.3) of feature 0 in layer activation (from test 84)
#1 BFC: 33.33333333% after failed attempt
…
| Targeting interval (-inf, -66.3) of feature 0 in layer activation (from test 35)
#9 BFC: 33.33333333% with new test case at Linf distance 0.10196081306420118: passed
| Targeting interval (-inf, -66.3) of feature 0 in layer activation (from test 102)
#10 BFC: 33.33333333% after failed attempt
Terminating after 10 iterations: 3 tests generated, 0 of which is adversarial.
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=6cm]{res/fm-medium-bfc-0-montage-5.png}%
  }\par
\end{frame}

\subsubsection{Feature-dependence Coverage with Concolic Search Engine (\(L_∞\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic dbnc fashion-mnist medium bfdc linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/bfdc-linf --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --bn-abstr outs/fm-medium/bn.pkl --criterion bfdc --norm linf --save-all-tests --init 100 --max-iterations 10
\end{cmds}
\begin{textcode}
Initializing with 100 randomly selected test cases that are correctly classified.
#0 BFdC: 81.39733333%
| Targeting interval [-41.5, -10.1] of feature 2 in layer activation_1, subject to feature intervals (1, 1, 1) in layer activation (from test 55)
#1 BFdC: 81.39733333% after failed attempt
…
| Targeting interval [-5.23, 25.5] of feature 1 in layer activation_1, subject to feature intervals (1, 3, 2) in layer activation (from test 1)
#5 BFdC: 86.20444444% with new test case at Linf distance 0.08235297086192112: passed
…
#10 BFdC: 86.66666667% after failed attempt
Terminating after 10 iterations: 2 tests generated, 0 of which is adversarial.
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=6cm]{res/fm-medium-bfdc-0-montage-9.png}%
  }\par
\end{frame}

\subsection{\DeepConcolic~--- Live Demos with HAR}

\input{har}

\subsubsection{Creating a BN Abstraction}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
\begin{cmds}
python3 -m deepconcolic.dbnabstr --dataset OpenML:har --model saved_models/har_dense.h5 create outs/har-dense/bn.pkl --feature-extraction pca --num-features 3 --num-intervals 3 --extended-discr --layers dense dense_{1,2,3} activation
\end{cmds}
\begin{textcode}
…
| Given 7724 classified training sample
| Extracting features for layer dense...
| Extracted 3 features
| Discretizing features for layer dense...
| Discretization of feature 0 involves 3 intervals
| Discretization of feature 1 involves 3 intervals
| Discretization of feature 2 involves 3 intervals
| Discretized 3 features
…
| Captured variance ratio for layer dense is 64.74%
| Captured variance ratio for layer dense_1 is 66.94%
| Captured variance ratio for layer dense_2 is 75.86%
| Captured variance ratio for layer dense_3 is 76.04%
| Captured variance ratio for layer activation is 61.03%
| Created Bayesian Network of 15 nodes and 36 edges.
Dumping abstraction into `outs/har-dense/bn.pkl'... done
\end{textcode}
\end{frame}

\subsubsection{Inspecting the BN Abstraction}
\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  % !deepconcolic dbnc show fashion-mnist medium pca
\begin{cmds}
python3 -m deepconcolic.dbnabstr --dataset OpenML:har --model saved_models/har_dense.h5 show outs/har-dense/bn.pkl
\end{cmds}
\begin{textcode}
===  Extracted Features and Associated Intervals  ==============================
Layer       Feature    Intervals
----------  ---------  -----------------------------------------
dense       0          (-inf, -15.6), [-15.6, 155), [155, inf)
            1          (-inf, -3.13), [-3.13, 375), [375, inf)
            2          (-inf, -11.7), [-11.7, 29.1), [29.1, inf)
dense_1     0          (-inf, -9.06), [-9.06, 15.6), [15.6, inf)
            1          (-inf, -6.52), [-6.52, 19.1), [19.1, inf)
            2          (-inf, -11.2), [-11.2, 13.5), [13.5, inf)
dense_2     0          (-inf, -8.43), [-8.43, 15.8), [15.8, inf)
            1          (-inf, -6.71), [-6.71, 14.2), [14.2, inf)
            2          (-inf, -5.83), [-5.83, 10.5), [10.5, inf)
dense_3     0          (-inf, -7.16), [-7.16, 12.6), [12.6, inf)
            1          (-inf, -5.08), [-5.08, 11), [11, inf)
            2          (-inf, -7.05), [-7.05, 8.23), [8.23, inf)
activation  0          (-inf, -1.61), [-1.61, 1.81), [1.81, inf)
            1          (-inf, -1.53), [-1.53, 1.69), [1.69, inf)
            2          (-inf, -1.44), [-1.44, 1.78), [1.78, inf)
\end{textcode}
\end{frame}

\subsubsection{Feature Coverage with ``Pixel''\-wise Optimisation (\(L_0\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic dbnc har dense bfc l0 single-seed
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/har-dense/bfc-l0-singleseed --dataset OpenML:har --model saved_models/har_dense.h5 --bn-abstr outs/har-dense/bn.pkl --criterion bfc --norm l0 --filters LOF --save-all-tests --max-iterations 100
\end{cmds}
\begin{textcode}
…
Initializing LOF-based novelty estimator with 3000 training samples... done
LOF-based novelty offset is -1.5
Starting tests for criterion BFC with norm L0 (1000 max iterations).
…
Randomly selecting an input from test data.
#0 BFC: 33.33333333%
| Targeting interval [1.78, inf) of feature 2 in layer activation (from test 0)
#1 BFC: 33.33333333% after failed attempt
…
| Targeting interval (-inf, -6.52) of feature 1 in layer dense_1 (from test 0)
#5 BFC: 33.33333333% with failed attempt at L0 distance 13: too far from original input
| Targeting interval [1.69, inf) of feature 1 in layer activation (from test 0)
#6 BFC: 33.33333333% after failed attempt
…
| Targeting interval [155, inf) of feature 0 in layer dense (from test 0)
#29 BFC: 33.33333333% after failed attempt
| Targeting interval [375, inf) of feature 1 in layer dense (from test 0)
#30 BFC: 33.33333333% after failed attempt
Unable to find a new candidate input!
Terminating after 30 iterations: 0 test generated, 0 of which is adversarial.
\end{textcode}
\end{frame}

% \begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% % !deepconcolic dbnc har dense bfc l0 init1000
% \begin{cmds}
% python3 -m deepconcolic.main --outputs outs/har-dense/bfc-l0-init100 --dataset OpenML:har --model saved_models/har_dense.h5 --bn-abstr outs/har-dense/bn.pkl --criterion bfc --norm l0 --filters LOF --save-all-tests --init 1000 --max-iterations 100
% \end{cmds}
% \begin{textcode}
% …
% Initializing with 1000 randomly selected test cases that are correctly classified.
% #0 BFC: 40.00000000%
% | Targeting interval (-inf, -1.61) of feature 0 in layer activation (from test 1)
% #1 BFC: 40.00000000% with new test case at L0 distance 1: passed
% | Targeting interval (-inf, -1.61) of feature 0 in layer activation (from test 3)
% #2 BFC: 40.00000000% with new test case at L0 distance 1: passed
% …
% | Targeting interval [375, inf) of feature 1 in layer dense (from test 100)
% #998 BFC: 88.88888889% after failed attempt
% | Targeting interval [375, inf) of feature 1 in layer dense (from test 120)
% #999 BFC: 88.88888889% after failed attempt
% | Targeting interval [375, inf) of feature 1 in layer dense (from test 119)
% #1000 BFC: 88.88888889% after failed attempt
% Terminating after 1000 iterations: 111 tests generated, 0 of which is adversarial.
% \end{textcode}
% \end{frame}

\subsubsection{Feature Coverage with Concolic Search Engine (\(L_∞\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  % !deepconcolic dbnc har dense bfc linf init100
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/har-dense/bfc-linf-init100 --dataset OpenML:har --model saved_models/har_dense.h5 --bn-abstr outs/har-dense/bn.pkl --criterion bfc --norm linf --filters LOF --save-all-tests --init 100 --max-iterations 100
\end{cmds}
\begin{textcode}
…
Initializing with 100 randomly selected test cases that are correctly classified.
#0 BFC: 88.88888889%
| Targeting interval (-inf, -15.6) of feature 0 in layer dense (from test 64)
#1 BFC: 88.88888889% after failed attempt
| Targeting interval (-inf, -15.6) of feature 0 in layer dense (from test 69)
#2 BFC: 88.88888889% with new test case at Linf distance 0.1043334704: passed
…
#98 BFC: 88.88888889% after failed attempt
| Targeting interval (-inf, -15.6) of feature 0 in layer dense (from test 31)
#99 BFC: 88.88888889% with new test case at Linf distance 0.0764798633: passed
| Targeting interval (-inf, -15.6) of feature 0 in layer dense (from test 112)
#100 BFC: 88.88888889% with failed attempt at Linf distance 0.08292110700000002: too far from original input
Terminating after 100 iterations: 13 tests generated, 0 of which is adversarial.
\end{textcode}
\end{frame}

% Local variables:
% TeX-master: "slides-deepconcolic-high-level"
% End:

% LocalWords:  Concolic activations


==> deepconcolic-high-level.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{High-level Coverage-guided Testing with \DeepConcolic}
\label{sec:deepconcolic-high-level}

\subsection{\DeepConcolic Overview (Recall from Session 2)}

\begin{frame}[label=deepconcolic-overview-high-level]{\insertsubsection}
  \centering
  \onslide<+->\input{fig/deepconcolic-overview}
  \vspace{2mm}
  \begin{minipage}{.58\linewidth}
    \begin{block}{%
        A \emph{search engine} seeks to increase a \emph{coverage metric}\\
        to achieve a \emph{test criterion}%
      }<+->
      \quad
      \usebeamertemplate{itemize item}
      Structural (Session 2)
      \hfill
      \usebeamertemplate{itemize item}
      \alert{High-level} (This session)
      \quad
    \end{block}
  \end{minipage}
  \vspace*{-1cm}
\end{frame}

\subsection{From Structural to High-level Coverage}

\begin{frame}{\insertsubsection}
  \begin{block}{Key Observations}
    Structural coverage metrics only reflect the low-level behaviours of neurons or pairs of neurons (\eg one neuron ≡ one condition)\\
    Issues:
    \begin{itemize}
    \item The very high number of neurons in typical DNNs impairs scalability of structural approaches
    \item We can question the adequacy of reasoning at the neuron level \wrt some higher level, assumed closer to the semantics of the data
    \end{itemize}
    One way forward:
    \begin{itemize}
    \item Leverage statistical analysis of neuron activations % induced by training data
      to discover high-level features learned by each hidden layer
    \end{itemize}
  \end{block}
\end{frame}

% \subsection{Key Concepts for High-level Coverage}
\subsection{High-level Coverage-guided Testing in \DeepConcolic}

\begin{frame}<1-2>[label=hl-testing]{\insertsubsection}
  \begin{block}{Overall Approach}
    Given a DNN \N, construct a \emph{Bayesian Network} (BN) to:
    \begin{itemize}
    \item Represent an abstraction of \emph{prominent behaviours} of \N
    \item Identify \emph{semantic assumptions} missed by test data
    \item[⤳] \emph{Define} and \emph{measure coverage} by using the BN
    \end{itemize}
  \end{block}
  \medskip
  \pause
  \begin{block}{Bayesian Network}
    Directed graph where:
    \begin{itemize}
    \item Each node denotes a \emph{categorical variable}
    \item Each edge represents a \emph{conditional dependency}
    \end{itemize}
  \end{block}
  % \medskip
  % \pause
  % \begin{block}{% Abstracting prominent behaviours with a
  %     BN-based Abstraction}
  %   \begin{itemize}
  %   \item Extract \emph{hidden features} learned by each hidden layer of \N
  %     % \item \emph{Partition} each hidden feature into a set of intervals
  %   \item[⤳] \emph{Partition} each hidden feature into a set of intervals
  %   \item[⤳] \emph{Connect} hidden features of successive layers
  %   \end{itemize}
  % \end{block}
% % \item Define \emph{coverage metrics} that measure how a test suite exercises hidden features
  % %   - Discretization of hidden feature domains (\(\featdom i ⤳ \DiscrFeatsSpace i\))
  % %   - Represent and measure cover
  % %   % \end{itemize}
  % %   % \begin{itemize}
  % %   % \item Extraction of Hidden Features via \emph{Dimensionality Reduction Techniques}
  % %   %   \begin{itemize}
  % Sequential nature of considered DNN \& discretised \HFs
  %   \begin{itemize}
  %   \item[⤳] Structure of a Bayesian Network (BN) where
  %   \item Each random variable represents a \HF and taking its values in the set of associated intervals
  %   \item Each edge represents an assumed causality relation between \HFs
  %   \end{itemize}
  % \begin{block}{Interpretation of the BN}
  % Use the BN to represent and measure coverage:
  %   \begin{itemize}
  %   \item a marginal probability
  %     shows how ``frequently'' \HF valuation belongs to some interval when the tests suite is fed to the DNN;
  %     % this tells how the interval is exercised by the test suite;
  %     % (\ie marginal probability of a variable taking an interval represents how frequent is this interval visited in the test suite)
  %   \item a conditional probability
  %     indicates how a causality assumption between hidden features of successive layers is exercised by the test suite (high-level counterpart of MC/DC)
  %   \end{itemize}
  % \end{block}
  % % \end{itemize}
  % % \end{block}
\end{frame}

\subsection{DNN Abstraction via Dimensionality Reduction}

% \subsection{Extraction of Hidden Features% via Dimensionality Reduction
% }

% \begin{frame}[label=dimred]{\insertsubsection}
%   % \begin{block}{Problem}<+->
%   % \begin{itemize}
%   % \item Given a layer with \(H\) neurons, and an input \(x\)
%   % \item A vector \(h(x) ∈ \RR^H\) describes
%   %   all activations at the layer % induced by % some input
%   %   % \(x\)
%   %   % where \(H\) is the number of neurons in \(l\)
%   % \item Problem: find a mapping λ that transforms \(h(x)\)\\
%   %   into a vector in \(\RR^L\), with \(L << H\)
%   %   % se a dimensionality reduction technique\\
%   %   % to deal with elements in \(\RR^L\) instead
%   %   \begin{itemize}
%   %   \item \(\RR^L\) is the \emph{hidden feature space} for the layer
%   %   \end{itemize}
%   %   % How can we deal with large
%   %   % Given \(h ∈ \RR^H\) a vector of all neuron activations
%   %   % induced by an input \(x\) at a given layer, we want to obtain an
%   %   % \mbox{\(L\)-dimensional} vector \(f ∈ \RR^L\) in some
%   % \end{itemize}
%   % \end{block}
%   \begin{block}{Principles}<+->
%     \begin{itemize}
%     \item Avoid dealing with the \(H\)-dimensional vectors of\\
%       activations induced by an input at a layer with \(H\) neurons
%     \item Use dimensionality reduction to obtain \(L\)-dimensional vectors
%     \end{itemize}
%   \end{block}
%   \begin{block}{\emph{Linear} Dimensionality Reduction of Activations \(h = l(x)\)}<+->
%     \begin{itemize}
%     \item
%       Compute \(W ∈ \RR^{H×L}\) and \(B ∈ \RR^L\) such that the mapping
%       \[λ\colon h ⟼ h W + B\]
%       projects any given \mbox{\(H\)-dimensional} vector \(h % = l(x)
%       ∈
%       \RR^H\) % (neuron activations)
%       into an \mbox{\(L\)-dimensional} space (with \(L << H\))
%     % \item \(x ∈ \RR^H\) is a vector of activations at a given layer of \(H\) neurons
%     \item \(\RR^L\) is the \emph{hidden feature space} for the layer
%     \end{itemize}
%   \end{block}
%   \begin{block}{Statistical approaches for computing \(W\) (and \(B\))}<+->
%     \begin{itemize}
%     \item Principal Component Analysis -- PCA:
%       % \begin{itemize}
%       % \item The resulting feature space
%       maximises the \emph{variance} in the data
%       % \end{itemize}
%     \item Independent Component Analysis -- ICA:
%       % \begin{itemize}
%       % \item The resulting feature space
%       identify \emph{statistically independent} signals
%       % \end{itemize}
%     \end{itemize}
%   \end{block}
% \end{frame}

\begin{frame}<1-6>[label=dbnabstr-overview]{\insertsubsection}
  \only<-11>{\input{fig/dbnabstr-overview.tikz}}%
  \only<12->{\input{fig/dbnabstr-overview-bn-constr.tikz}\vspace{3cm}}%
\end{frame}

\begin{heavypgf}
  \subsubsection{Extraction of Hidden Features with \emph{PCA}}

  \begin{frame}{\insertsubsubsection}
    \begin{block}{2 \HFs extracted from a layer \(\mathtt{dense}\)}
      \vspace{2mm}
      \resizebox{.7\textwidth}{!}{\inputpgf{fig/fashion_mnist-dense-pca-2d}}
    \end{block}
  \end{frame}

  \subsubsection{Extraction of Hidden Features with \emph{ICA}}

  \begin{frame}{\insertsubsubsection}
    \begin{block}{2 \HFs extracted from a layer \(\mathtt{dense}\)}
      \vspace{2mm}
      \resizebox{.7\textwidth}{!}{\inputpgf{fig/fashion_mnist-dense-ica-2d}}
    \end{block}
  \end{frame}
\end{heavypgf}

% \begin{frame}{Hidden Features}
%   \vspace{3mm}
%   \begin{block}{2 \HFs extracted from a layer \layer{\mathtt{dense}}}
%     \vspace{2mm}
%     \largepgf{\resizebox{.9\textwidth}{!}{\input{fig/mnist_small-dense-dens-nosplit.pgf}}}
%   \end{block}
% \end{frame}

\subsection{Discretisation of Hidden Features}

\againframe<7-11>{dbnabstr-overview}

\begin{frame}{\insertsubsection}{Example for 2 Hidden Features}
  \centering
  \resizebox{.96\textwidth}{!}{\input{fig/mnist_small-dense-dens.pgf}}
  \begin{itemize}
  \item For our demos we only use a uniform discretisation strategy
  \end{itemize}
\end{frame}

\subsection{Construction of the Bayesian Network}

\againframe<12->{dbnabstr-overview}

% \againframe<2->{hl-testing}
% {\usebackgroundtemplate{\centering\includegraphics[width=.9\textwidth]{fig/example-BN.png}}
\begin{frame}{\insertsubsection~-- Example \BNa\N X}
  \centering
  \includegraphics[width=.9\textwidth]{fig/example-BN.png}
\end{frame}


\subsection{BN-based Coverage-guided Testing}

\begin{frame}{\insertsubsection}
  % \begin{block}{Construction of the Bayesian Network}<+->
  %   \begin{itemize}
  %   \item Given a DNN \N, a BN structure \BN\N{∅}, and a test suite \(X\)
  %   \item Compute probabilities in the BN \BN\N X via Bayesian Inference
  %   \end{itemize}
  % \end{block}
  \begin{block}{Coverage Metrics}<+->
    \begin{enumerate}
    \item Feature coverage -- \BNFCov\N X\par
      \raggedleft ⤳ Proportion of marginal probabilities \(\approx 0\)
      \par\raggedright
    \item Feature-dependence coverage -- \BNFxCov\N X\par
      \raggedleft ⤳ Proportion of conditional probabilities \(\approx 0\)\\
      (subject to marginal probability \(> 0\))
      \par\raggedright
    \end{enumerate}
  \end{block}
  \medskip
  \begin{block}{Selecting Test Targets}<+->
    \begin{itemize}
    \item Feature coverage: identify an entry with
      a marginal probability \(\approx 0\)
    \item Feature-dependence coverage: identify an entry with
      a conditional probability \(\approx 0\)
    % \item Then search for a candidate input \(x\) that is close to
    \end{itemize}
  \end{block}
\end{frame}

\subsection{Exploiting the BN Abstraction}

\begin{frame}{\insertsubsection}
  \begin{block}{Concolic Testing}<+->
    \begin{itemize}
    \item Given a target interval \(\I_{i,j}\) for the \HF \(j\) at a layer \layer i and candidate input \(x\)
    \item Perform symbolic analysis to find \(x'\):
      \begin{enumerate}
      \item Pixel\-wise optimisation for \(L_0\) exploration (exhaustive search)
      \item Use a Linear Programme (LP) for \(L_∞\) exploration:
      \item[] Minimise \LInf x {x'}
      \item[] Subject to constraints that encode the behaviour of \(\N(x)\)
      \item[] \emph{and}
        \(（\mathsf{discr}^{♯}_i∘λ_i∘\layer i ∘ ⋯ ∘ \layer 1(x')）_j ∈ \I_{i,j}% \subfeatspace l i k
        \)
      \end{enumerate}
      \hfill ⤳ Requires the \(λ_i\)'s to be \emph{linear} (\eg computed via PCA or ICA)
    \end{itemize}
  \end{block}
  \begin{block}{Further Uses}<+->
  \begin{itemize}
  \item Probabilistic inference
  \item Runtime monitoring
  \end{itemize}
  \end{block}
  \medskip
  \begin{itemize}
  \item \red{Now, off for the tool demo …}
  \end{itemize}
  % \begin{block}{Concolic search engine for \(L_∞\) norm exploration}<+->
  %   \begin{itemize}
  %   \item To target the interval % \subfeatspace l i k
  %     \(\I_{i,j}\) for the \HF \(j\) at a layer \layer i, given a candidate input \(x\):
  %     \begin{enumerate}
  %     % \item Construct an LP encoding the behaviours of \(\N(x\) up to \layer i
  %       % \item Encode the linear mapping \(λ_{l,i}\) that defines the \HF i of layer \(l\)
  %     % \item Minimise \LInf x {x'} subject to additional constraints \(λ_{l,i}(l(x')) ∈ \subfeatspace l i k\)
  %     \item Minimise
  %     \item[] Subject to constraints that encode the behaviour of \(\N(x)\) up to layer \layer i, \emph{and}
  %       \)
  %       % \par
  %       % \raggedleft
  %       % (\(λ_{l,i}\) is a linear mapping that defines the \HF i of layer \(l\))
  %     \end{enumerate}
  %     \hfill ⤳ requires the \(λ_i\)'s to be \emph{linear}
  %   \item
  %     (A similar approach allows to target the feature-dependence criterion)
  %   \end{itemize}
  % \end{block}
  % \smallskip
  % \begin{block}{Pixel\-wise optimisation for \(L_0\) exploration}<+->
  %   \begin{itemize}
  %   \item Exhaustive search by direct manipulation of input features from
  %     \(x\) also allows to target feature coverage
  %   \end{itemize}
  % \end{block}
\end{frame}

% Local variables:
% TeX-master: "slides-deepconcolic-high-level"
% End:

% LocalWords:  activations Discretisation upto Concolic discretised
% LocalWords:  discretisation


==> deepconcolic-structural-demo.tex <==
% -*- coding: utf-8; mode: latex -*-

\subsection{Relevant Command-line Options}

\begin{frame}[allowframebreaks]{\insertsubsection}
  \begin{block}{General}
    \begin{itemize}
    \item \shparambox{--dataset $D$ --model $\mathit{DNN}$}
      (as for \shparambox{deepconcolic.eval\_classifier})
    \item \shparambox{--outputs $\mathit{directory}$},
      \shparambox{--init $|X_0|$}, \shparambox{--max-iterations $N$},
      \shparambox{--save-all-tests}
    \end{itemize}
  \end{block}
  \begin{block}{Exploration}
    \begin{itemize}
    \item Norm for Oracle and Search Engine: \shparambox{--norm \{l0,linf\}}
    \item Test Criterion: \shparambox{--criterion \{nc, ssc, ssclp\}}
    \item Layer selection: \shparambox{--layers $\mathit{layer~names}$}
    \end{itemize}
  \end{block}
  \begin{exampleblock}{Examples}
    \begin{itemize}
    \item \(L_0\) exploration for NC: \shparambox{--norm l0 --criterion nc}
    \item \(L_∞\) exploration via concolic testing for NC: \shparambox{--norm linf --criterion nc}
    \item \(L_∞\) exploration via gradient analysis for SSC: \shparambox{--norm linf --criterion ssc}
    \item \(L_∞\) exploration via concolic testing for SSC: \shparambox{--norm linf --criterion ssclp}
    \end{itemize}
  \end{exampleblock}
  \framebreak
  \begin{block}{Oracle}
    \begin{itemize}
    \item Distance threshold for the oracle: \shparambox{--norm-factor $\dthr$}
    \item[] (defaults to \(\frac 1 4\) for \(L_∞\), \(\frac{|\mbox{input features}|} 4\) for \(L_0\))
    \item Outlier/novelty detection for non-image data: \shparambox{--filters LOF}
    \end{itemize}
  \end{block}
  \begin{block}{Concolic Testing% (\(L_∞\) norm)
    }
    \begin{itemize}
    \item Hard lower-bound for \(\|x - x'\|_∞\): \shparambox{--lb-hard $\dminHard$}
      \hfill(\(\dminHard ∈ [0,1[\))
    \item Noise for the lower-bound of \(\|x - x'\|_∞\): \shparambox{--lb-noise $\dminNoise$}
      \hfill(\(\dminNoise ∈ [0,1-\dminHard[\))
    \item Enforce \(\|x-x'\|_∞ ≥ \dminHard + d'\), with \(d' \sim U(0,\dminNoise)\)
    \end{itemize}
  \end{block}
  \begin{block}{Gradient Analysis}
    \begin{itemize}
    \item \shparambox{--mcdc-cond-ratio $r$} consider activations of a ratio $r$ of neurons in condition layers (instead of a single neuron)\hfill (defaults to \(\frac 1 {100}\))
    \end{itemize}
  \end{block}
\end{frame}

% \section{Live Demos of \DeepConcolic}

\subsection{\DeepConcolic --- Live Demos with Fashion-MNIST}

\input{dc-update}

\input{fm}

\subsubsection{Training or Downloading a Suitable Model}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  \begin{block}{Training}
% !train deepconcolic fashion-mnist dense medium large
\begin{cmds}
mkdir -p gentmp saved_models
TMPDIR=$PWD/gentmp python3 -m deepconcolic.gen_fashion_mnist
mv gentmp/fashion_mnist_{medium,large}.h5 saved_models/
\end{cmds}
  \end{block}
  \begin{block}{Downloading}
% !silent download deepconcolic fashion-mnist dense medium large
\begin{cmds}
wget -P saved_models https://cgi.csc.liv.ac.uk/~acps/models/fashion_mnist_medium.h5
wget -P saved_models https://cgi.csc.liv.ac.uk/~acps/models/fashion_mnist_large.h5
\end{cmds}
  \end{block}
\end{frame}

\subsubsection{Neuron Coverage with Pixel\-wise Optimisation (\(L_0\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic nc fashion-mnist medium l0
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/nc-l0 --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --layers activation activation_1 activation_2 --criterion nc --norm l0 --save-all-tests --max-iterations 100
\end{cmds}
\begin{textcode}
Randomly selecting an input from test data.
#0 NC: 36.49130629%
| Targeting activation of (1, 4, 27) in conv2d
#1 NC: 36.95942934% with new test case at L0 distance 1: passed
…
| Targeting activation of (23, 4, 12) in conv2d
#63 NC: 50.53499777% with new test case at L0 distance 1: adversarial
…
| Targeting activation of (19, 11, 15) in conv2d
#100 NC: 56.94010997% with new test case at L0 distance 1: passed
Terminating after 100 iterations: 92 tests generated, 4 of which are adversarial.
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=6cm]{res/fm-medium-nc-l0-0-montage-3.png}%
  }\par
\end{frame}

\subsubsection{Neuron Coverage with Concolic Search Engine (\(L_∞\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  \begin{itemize}
  \item First activation layer of \inlinesh{fashion_mnist_medium.h5}, with \(|X_0| = 1\)
  \end{itemize}
% !deepconcolic nc fashion-mnist medium linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/nc-linf --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --layers activation --criterion nc --norm linf --save-all-tests --max-iterations 10
\end{cmds}
  \centering%
  \vspace*{-4mm}%
  \montagebox{%
    \includegraphics[width=6cm]{res/fm-medium-nc-linf-0-montage-6.png}%
  }\par
  \pause\bigskip
  \begin{itemize}
  \item All activation layers of \inlinesh{fashion_mnist_large.h5}, with \(|X_0| = 100\)
  \end{itemize}
% !deepconcolic nc fashion-mnist medium linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-large/nc-linf --dataset fashion_mnist --model saved_models/fashion_mnist_large.h5 --criterion nc --norm linf --save-all-tests --max-iterations 10 --init 100
\end{cmds}
\end{frame}

\subsubsection{Sign-Sign Coverage with Concolic Search Engine}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  \begin{itemize}
  \item Testing \inlinesh{fashion_mnist_medium.h5}
  \item Conditions layer: \inlinesh{activation}
  \item Decisions layer: \inlinesh{activation\_1}
  \end{itemize}
% !deepconcolic ssclp fashion-mnist medium linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/ssclp-linf --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --layers activation_1 --criterion ssclp --norm linf --save-all-tests --max-iterations 10
\end{cmds}
\begin{textcode}
…
Considering 4147200(/4147200) neuron pairs w.r.t decision layer conv2d_1
…
Base LP encoding of DNN fashion_mnist_medium_maxp up to layer 4 has 59824 variables.
Base LP encoding of deepest layer considered involves 50016 constraints.
Starting tests for criterion SSC with norm Linf (10 max iterations).
…
Randomly selecting an input from test data.
#0 SSC: 0.00000000%
…
| Targeting decision (6, 7, 36) in conv2d_1, subject to condition (9, 7, 20) in conv2d
#10 SSC: 0.00024113% with new test case at Linf distance 0.015686274509803977: passed
Terminating after 10 iterations: 10 tests generated, 0 of which is adversarial.
\end{textcode}
\end{frame}

\subsubsection{Sign-Sign Coverage with Gradient Analysis}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  \begin{itemize}
  \item Testing \inlinesh{fashion_mnist_medium.h5}
  \item Conditions layer: \inlinesh{activation}
  \item Decisions layer: \inlinesh{activation\_1}
  \item Loosened definition of sign-sign coverage (\shparambox{--mcdc-cond-ratio 0.1})
  \end{itemize}
% !deepconcolic ssc fashion-mnist medium linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/fm-medium/ssc-linf --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5 --layers activation_1 --criterion ssc --norm linf --mcdc-cond-ratio 0.1 --save-all-tests --max-iterations 3
\end{cmds}
\begin{textcode}
…
Considering 4147200(/4147200) neuron pairs w.r.t decision layer conv2d_1
…
#0 SSC: 0.00000000%
| Targeting decision (2, 2, 25) in conv2d_1, subject to any condition
#1 SSC: 0.01929012% with new test case at Linf distance 0.007843165304146527: passed
| Targeting decision (1, 4, 4) in conv2d_1, subject to any condition
#2 SSC: 0.03858025% with new test case at Linf distance 0.003921592469308899: passed
| Targeting decision (8, 3, 15) in conv2d_1, subject to any condition
#3 SSC: 0.05787037% with new test case at Linf distance 0.0039215980791578176: passed
Terminating after 3 iterations: 3 tests generated, 0 of which is adversarial.
\end{textcode}
\end{frame}

\subsection{Live Demos with HAR}

\input{har}

\subsubsection{Training or Downloading a Suitable Model}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  \begin{block}{Training}
% !train deepconcolic har dense decomposed
\begin{cmds}
mkdir -p gentmp saved_models
TMPDIR=$PWD/gentmp python3 -m deepconcolic.gen_har
mv gentmp/har_dense_decomposed.h5 gentmp/har_dense.h5 saved_models/
\end{cmds}
  \end{block}
  \begin{block}{Downloading}
\begin{cmds}
wget -P saved_models https://cgi.csc.liv.ac.uk/~acps/models/har_dense_decomposed.h5
\end{cmds}
% mkdir -p saved_models
% wget -O saved_models/har_dense_decomposed.h5 "https://www.dropbox.com/s/cf5gvkv9k0wtlux/har_dense_decomposed.h5?dl=0"
  \end{block}
\end{frame}

\subsubsection{Neuron Coverage with Feature\-wise Optimisation (\(L_0\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic nc har dense decomposed l0
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/har-dense-decomposed/nc-l0 --dataset OpenML:har --model saved_models/har_dense_decomposed.h5 --layers activation activation_{1,2,3} --criterion nc --norm l0 --save-all-tests --max-iterations 100 --init 100 --filters LOF
\end{cmds}
\begin{textcode}
…
DNN under test has 11 layer functions, 4 of which are to be covered:
[dense, dense_1, dense_2, dense_3]
…
Initializing LOF-based novelty estimator with 3000 training samples... done
LOF-based novelty offset is -1.5
…
Starting tests for criterion NC with norm L0 (100 max iterations).
Initializing with 100 randomly selected test cases that are correctly classified.
#0 NC: 74.36974790%
| Targeting activation of 167 in dense
…
#99 NC: 75.00000000% with failed attempt at L0 distance 8: too far from original input
| Targeting activation of 14 in dense
#100 NC: 75.00000000% with failed attempt at L0 distance 9: too far from original input
Terminating after 100 iterations: 3 tests generated, 0 of which is adversarial.
\end{textcode}
\end{frame}

\subsubsection{Visualising HAR Test Cases}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
  \begin{itemize}
  \item Selection of 32 features
  \end{itemize}
\begin{cmds}
DC_MPL_BACKEND=pgf DC_MPL_FIG_RATIO=.5 python3 -m utils.harviz --features 32 outs/har-dense-decomposed/nc-l0 --outputs outs/har-dense-decomposed/nc-l0
\end{cmds}
  \smallskip
  \centering
  \resizebox{.8\linewidth}{!}{\inputpgf{fig/har-smpl-l0}}
  \par
\end{frame}

\subsubsection{Neuron Coverage with Concolic Search (\(L_∞\) Norm)}

\begin{frame}[fragile]{\insertsubsubsection}{\insertsubsection}
% !deepconcolic nc har dense decomposed linf
\begin{cmds}
python3 -m deepconcolic.main --outputs outs/har-dense-decomposed/nc-linf --dataset OpenML:har --model saved_models/har_dense_decomposed.h5 --layers activation activation_{1,2,3} --criterion nc --norm linf --save-all-tests --max-iterations 10 --init 100 --filters LOF
\end{cmds}
\begin{textcode}
…
DNN under test has 11 layer functions, 4 of which are to be covered:
[dense, dense_1, dense_2, dense_3]

…
Starting tests for criterion NC with norm Linf (10 max iterations).
…
Initializing with 100 randomly selected test cases that are correctly classified.
#0 NC: 74.57983193%
| Targeting activation of 136 in dense
#1 NC: 74.57983193% with failed attempt at Linf distance 0.10202241000000006: too far from original input
| Targeting activation of 178 in dense
#2 NC: 74.78991597% with new test case at Linf distance 0.05494287100000002: passed
| Targeting activation of 57 in dense
…
#9 NC: 75.42016807% with new test case at Linf distance 0.0210680304: passed
| Targeting activation of 136 in dense
#10 NC: 75.42016807% with failed attempt at Linf distance 0.06752224000000007: too far from original input
Terminating after 10 iterations: 4 tests generated, 0 of which is adversarial.
\end{textcode}
\end{frame}

% Local variables:
% TeX-master: "slides-session2"
% End:

% LocalWords:  Concolic activations


==> deepconcolic-structural.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Structural Coverage-guided Testing with \DeepConcolic}
\label{sec:deepconcolic-structural}

\subsection{\DeepConcolic Overview}

\begin{frame}<1>[label=deepconcolic-overview-structural]{\insertsubsection}
  \centering
  \onslide<+->\input{fig/deepconcolic-overview}
  \vspace{2mm}
  \begin{minipage}{.58\linewidth}
    \begin{block}{%
        A \emph{search engine} seeks to increase a \emph{coverage metric}\\
        to achieve a \emph{test criterion}%
      }<+->
      \quad
      \usebeamertemplate{itemize item}
      \alert{Structural} (This session)
      \hfill
      \usebeamertemplate{itemize item}
      High-level (Session 5)
      \quad
    \end{block}
  \end{minipage}
  \vspace*{-1cm}
\end{frame}

\subsection[DNNs]{Deep Neural Networks (DNNs)}

\begin{frame}[fragile]{Deep Neural Networks (DNNs)}
  \begin{columns}
    \begin{column}{0.5\textwidth}<+->
      % \vspace{-0.8cm}
      \begin{figure}[htp!]
        \centering

        \def\layersep{1.8cm}

        \scalebox{0.8}{
        \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
            \tikzstyle{every pin edge}=[<-,shorten <=1pt]
            \tikzstyle{neuron}=[circle,fill=black!25,minimum size=20pt,inner sep=0pt]
            \tikzstyle{input neuron}=[neuron, fill=green!50];
            \tikzstyle{output neuron}=[neuron, fill=red!50];
            \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
            \tikzstyle{annot} = [text width=4em, text centered]

            % Draw the input layer nodes
            \foreach \name / \y in {1,...,2}
            % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
                \node[input neuron, pin=left:$ $] (I-\name) at (0,-\y) {};
                %\node[input neuron, pin=left:$v_{1,\y}$] (I-\name) at (0,-\y) {};
                %\node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

            % Draw the 1st hidden layer nodes
            \foreach \name / \y in {1,...,3}
                \path[yshift=0.5cm]
                    node[hidden neuron, draw=black, line width=2pt] (H1-\name) at (\layersep,-\y cm) {};

            % Draw the 2nd hidden layer nodes
            \foreach \name / \y in {1,...,2}
                \path[yshift=0.5cm]
                    node[hidden neuron] (H2-\name) at (\layersep*2,-\y cm) {};

            \foreach \name / \y in {3}
                \path[yshift=0.5cm]
                    node[hidden neuron, draw=black, line width=2pt] (H2-\name) at (\layersep*2,-\y cm) {};

            % Draw the output layer node
            \node[output neuron,pin={[pin edge={->}]right:$u_{4,1}$}, right of=H2-2, yshift=0.5cm] (O1) {};
            \node[output neuron,pin={[pin edge={->}]right:$u_{4,2}$}, right of=H2-2, yshift=-0.5cm] (O2) {};

            % Connect every node in the input layer with every node in the
            % hidden layer.
            \foreach \source in {1,...,2}
                \foreach \dest in {1,...,3}
                    \path (I-\source) edge (H1-\dest);

            \foreach \source in {1,...,3}
                \foreach \dest in {1,...,2}
                    \path (H1-\source) edge (H2-\dest);

            \foreach \source in {1,...,3}
                \foreach \dest in {3}
                    \draw[black, line width=2pt] (H1-\source) -- (H2-\dest);
                    %\path (H1-\source) edge (H2-\dest);


            \foreach \source in {1,...,3}
                 \path (H2-\source) edge (O1);

            \foreach \source in {1,...,3}
                 \path (H2-\source) edge (O2);

            % Annotate the layers
            \node[annot,above of=H1-1, node distance=1cm] (hl1) {Hidden layer};
            \node[annot,above of=H2-1, node distance=1cm] (hl2) {Hidden layer};
            \node[annot,left of=hl1] {Input layer};
            \node[annot,right of=hl2] {Output layer};

            \node[annot, right of=H1-1, node distance=0.0cm] (hl1) {\small $n_{2,1}$};
            \node[annot, right of=H1-2, node distance=0.0cm] (hl1) {\small $n_{2,2}$};
            \node[annot, right of=H1-3, node distance=0.0cm] (hl1) {\small $n_{2,3}$};
            \node[annot, right of=H2-1, node distance=0.0cm] (hl1) {\small $n_{3,1}$};
            \node[annot, right of=H2-2, node distance=0.0cm] (hl1) {\small $n_{3,2}$};
            \node[annot, right of=H2-3, node distance=0.0cm] (hl1) {\small $n_{3,3}$};
        \end{tikzpicture}
        }
        \end{figure}
        % \vspace{-0.5cm}
        \smallskip
        \[\mathit{label}=\argmax_{1\leq l\leq s_K}u_{K,l}\]
  \end{column}
  \begin{column}{0.5\textwidth}<+->
  1) neuron activation value
  \begin{equation*}
    \label{eq:sum}
    \begin{aligned}
      %  % &\mbox{\small 1) neuron activation value} \\
      &{{u_{k,i}}=b_{k,i}+\sum_{1\leq h \leq s_{k-1}} {w_{k-1, h, i}\cdot {v_{k-1,h}}}}\\
      &\mbox{\scriptsize --- weighted sum plus a bias; } \\
      &\mbox{\scriptsize --- w,b are parameters learned}\\
    \end{aligned}
  \end{equation*}

  % \begin{column}{0.5\textwidth}
  2) rectified linear unit (ReLU):
  $$\hspace*{-2.5cm}{v_{k,i}}=  \max\{{u_{k,i}}, 0\}$$
\end{column}
\end{columns}
\end{frame}

\begin{frame}[fragile]
  \frametitle{DNN as a program}
  \onslide<+->\begin{lstlisting}[mathescape=true]
    ...

    // 1) neuron activation value
    double $u_{k,i}$ = $\color{red}\mathbf{b_{k,i}}$;
    for (unsigned $h$ = $\color{cyan}1$; $h$ <= $s_{k-1}$; $h$ += $\color{cyan}1$)
    {
      $u_{k,i}$ += $\color{red}w_{k-1,h,i}$ * $v_{k-1,h}$;
    }

    double $v_{k,i}$ = $\color{cyan}0$;

    // 2) ReLU
    if ($u_{k,i}$ > $\color{cyan}0$)
    {
      $v_{k,i}$ = $u_{k,i}$;
    }

    ...
  \end{lstlisting}
  \tikz[overlay, remember picture]%
  \node<+->[xshift = -5cm, yshift = -2cm] at (current page.east) {%
    \begin{tcolorbox}[center, boxsep=0pt, left=1ex, right=1ex, width = 8cm, before upper=\strut, tcbox width = minimum center, box align=base, halign=left, colback=white!96!black]
      % \raggedright
      DNNs are complex non-linear functions
      with algorithmically generated (and not engineered) coefficients, and therefore are effectively “black boxes”.
    \end{tcolorbox}%
  };
\end{frame}

\subsection{DNN Coverage}

\begin{frame}{Coverage}
\begin{itemize}
    \item Coverage metrics provide a means to assess how much of the code is covered; increasing the coverage over the code means more tests, exercising more code.
    \begin{itemize}
        \item Provides increased confidence that sufficient testing has been undertaken.
        \item The more granular the coverage, the more tests likely to be required.
    \end{itemize}
    \item Coverage metrics for DNNs can’t use traditional approach: we need something more…
\end{itemize}
\end{frame}

\begin{frame}[fragile]
  \frametitle{Neuron coverage}
  \lstset{escapechar=@}
  \bigskip
  % \begin{columns}
  %   \begin{column}{0.49\textwidth}

  %     For any hidden neuron $n_{k,i}$, there exists a test case $t\in \testsuites$ such that the neuron
  %     $n_{k,i}$ is activated: $u_{k,i}>0$.
  %     $ap[t]_{k,i} = \true$.

  %     \vspace{2cm}
  %     \bigskip
  %     \bigskip
  %   \end{column}

  %   \begin{column}{0.575\textwidth}
  %     \vspace{-0.7cm}
  \begin{itemize}
  \item  $\approx$ statement (line) coverage
  \item For any hidden neuron $n_{k,i}$, there exists a test case $t$ such that the neuron
    $n_{k,i}$ is activated: $u_{k,i}>0$.
  \end{itemize}
  \vspace*{-5mm}
  \begin{center}
    \begin{minipage}{.5\linewidth}
      \begin{lstlisting}[mathescape=true]
    ...

    // 1) neuron activation value
    double $u_{k,i}$ = $b_{k,i}$;
    for (unsigned $h$ = $\color{cyan}1$; $h$ <= $s_{k-1}$; $h$ += $\color{cyan}1$)
    {
      $u_{k,i}$ += $\color{red}w_{k-1,h,i}$ * $v_{k-1,h}$;
    }

    double $v_{k,i}$ = $\color{cyan}0$;

    // 2) ReLU
    if ($u_{k,i}$ > $\color{cyan}0$)
    {
      @{\colorbox{blue!30}{$v_{k,i}$ = $u_{k,i}$;}}  ${\color{red}\mbox{  }\Leftarrow\mbox{{this line is covered}}}$@
    }

    ...
  \end{lstlisting}
\end{minipage}
\end{center}
\end{frame}

\begin{frame}{MC/DC (Modified Condition / Decision Coverage)}

  \begin{itemize}
  \item
    Developed by NASA and has been widely adopted in e.g., avionics software development guidance to ensure adequate testing of applications with the highest criticality.
    \bigskip
  \item Intent: if a choice can be made, all the possible factors (conditions) that contribute to that choice (decision) must be tested.
  \end{itemize}


\end{frame}

\begin{frame}[fragile]
\frametitle{MC/DC variant for DNNs}
\begin{columns}
\begin{column}{0.9\textwidth}
  %\vspace{-0.8cm}
  \begin{figure}[htp!]
    \centering

    \def\layersep{1.8cm}

    \scalebox{0.8}{
    \begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
        \tikzstyle{every pin edge}=[<-,shorten <=1pt]
        \tikzstyle{neuron}=[circle,fill=black!25,minimum size=20pt,inner sep=0pt]
        \tikzstyle{input neuron}=[neuron, fill=green!50];
        \tikzstyle{output neuron}=[neuron, fill=red!50];
        \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
        \tikzstyle{annot} = [text width=4em, text centered]

        % Draw the input layer nodes
        %\foreach \name / \y in {1,...,2}
        % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        %    \node[input neuron, pin=left:$ $] (I-\name) at (0,-\y) {};
            %\node[input neuron, pin=left:$v_{1,\y}$] (I-\name) at (0,-\y) {};
            %\node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

        % Draw the 1st hidden layer nodes
        \foreach \name / \y in {1,...,3}
            \path[yshift=0.5cm]
                node[hidden neuron, draw=black, line width=2pt] (H1-\name) at (\layersep,-\y cm) {};

        % Draw the 2nd hidden layer nodes
        %\foreach \name / \y in {1,...,2}
        %    \path[yshift=0.5cm]
        %        node[hidden neuron] (H2-\name) at (\layersep*2,-\y cm) {};

        \foreach \name / \y in {3}
            \path[yshift=0.5cm]
                node[hidden neuron, draw=black, line width=2pt] (H2-\name) at (\layersep*2,-\y cm) {};

        % Draw the output layer node
        %\node[output neuron,pin={[pin edge={->}]right:$u_{4,1}$}, right of=H2-2, yshift=0.5cm] (O1) {};
        %\node[output neuron,pin={[pin edge={->}]right:$u_{4,2}$}, right of=H2-2, yshift=-0.5cm] (O2) {};

        % Connect every node in the input layer with every node in the
        % hidden layer.
        %\foreach \source in {1,...,2}
        %    \foreach \dest in {1,...,3}
        %        \path (I-\source) edge (H1-\dest);

        %\foreach \source in {1,...,3}
        %    \foreach \dest in {1,...,2}
        %        \path (H1-\source) edge (H2-\dest);

        \foreach \source in {1,...,3}
            \foreach \dest in {3}
                \draw[black, line width=2pt] (H1-\source) -- (H2-\dest);
                %\path (H1-\source) edge (H2-\dest);


        %\foreach \source in {1,...,3}
        %     \path (H2-\source) edge (O1);

        % \foreach \source in {1,...,3}
        %     \path (H2-\source) edge (O2);

        % Annotate the layers
        \node[annot,above of=H1-1, node distance=1cm] (hl1) {Condition neurons};
        \node[annot,above of=H2-1, node distance=1cm] (hl2) {Decision neuron};
        %\node[annot,left of=hl1] {Input layer};
        %\node[annot,right of=hl2] {Output layer};

        \node[annot, right of=H1-1, node distance=0.0cm] (hl1) {\small $n_{2,1}$};
        \node[annot, right of=H1-2, node distance=0.0cm] (hl1) {\small $n_{2,2}$};
        \node[annot, right of=H1-3, node distance=0.0cm] (hl1) {\small $n_{2,3}$};
        %\node[annot, right of=H2-1, node distance=0.0cm] (hl1) {\small $n_{3,1}$};
        %\node[annot, right of=H2-2, node distance=0.0cm] (hl1) {\small $n_{3,2}$};
        \node[annot, right of=H2-3, node distance=0.0cm] (hl1) {\small $n_{3,3}$};
    \end{tikzpicture}
    }
    \end{figure}
        %\vspace{-0.5cm}

For each condition / decision pair e.g. $(n_{2,1}, n_{3,3})$, there are 4 test conditions
\begin{enumerate}
    \item condition $n_{2,1}$ is on, decision $n_{3,3}$ is on
    \item condition $n_{2,1}$ is on, decision $n_{3,3}$ is off
    \item condition $n_{2,1}$ is off, decision $n_{3,3}$ is on
    \item condition $n_{2,1}$ is off, decision $n_{3,3}$ is off
\end{enumerate}
\end{column}

\begin{column}{0.1\textwidth}

%For each condition / decision pair e.g. $(n_{2,1}, n_{3,3})$, there are 4 test conditions
%\begin{enumerate}
%    \item condition $n_{2,1}$ is on, decision $n_{3,3}$ is on
%    \item condition $n_{2,1}$ is on, decision $n_{3,3}$ is off
%    \item condition $n_{2,1}$ is off, decision $n_{3,3}$ is on
%    \item condition $n_{2,1}$ is off, decision $n_{3,3}$ is off
%\end{enumerate}

\end{column}

\end{columns}
\bigskip
multiple ways to define ``on/off'' (ss, vs, sv, vv)

neuron pair $\Rightarrow$ feature pair
\end{frame}

\begin{frame}{A summary of coverage metrics for testing DNNs}
  \centering%
  \only<+>{\includegraphics[width=0.95\linewidth]{images/coverage/relation.png}}%
  \only<+>{\includegraphics[width=0.95\linewidth]{images/coverage/relationship-nc.png}}%
  \only<+>{\includegraphics[width=0.95\linewidth]{images/coverage/relationship-nbc.png}}%
  \only<+>{\includegraphics[width=0.95\linewidth]{images/coverage/relationship-path.png}}%
  \only<+>{\includegraphics[width=0.95\linewidth]{images/coverage/relationship-mcdc.png}}%
\end{frame}

\subsection{Testing CNNs with \DeepConcolic}

\againframe<1->{deepconcolic-overview-structural}

\subsubsection{Test Loop}

\begin{frame}{\insertsubsection~-- \insertsubsubsection}
  \begin{block}{Test Criterion}
    \begin{itemize}
    \item Defines and measures coverage (\eg Neuron Coverage (NC), Sign Sign Change (SSC))
    \item Selects new test targets
    \item[] (and associated candidate inputs for concolic testing)
    \end{itemize}
  \end{block}
  \begin{block}{Search Engine}
    \begin{itemize}
    \item Given a test target \(t\) (\eg neuron to activate)
    \item[] and a candidate input \(x\) (for concolic testing):
    \item Generates a new input \(x'\) such that \(t\) is met
    % \item[] (Note \(x\) may have itself be derived from an original input taken from the raw data)
    \end{itemize}
  \end{block}
  \begin{block}{Oracle}
    \begin{itemize}
    \item Determines plausibility of generated inputs
    \item Checks if the DNN passes the oracle
    \end{itemize}
  \end{block}
\end{frame}

\subsubsection{Oracle}

\begin{frame}{\insertsubsection~-- \insertsubsubsection}
  \begin{block}{Determining Plausibility}
    \begin{itemize}
    \item Measuring a \emph{distance} between inputs, \wrt a given \emph{norm} \(L_p\) % \(\|x - x'\|_p\)
    \item Rejects any new input \(x'\) if \(\|x - x'\|_p > \dthr\), for some given threshold \dthr
    \end{itemize}
  \end{block}
  \begin{block}{In \DeepConcolic}<2->
    \begin{itemize}
    \item<1-> \(L_0\) -- \emph{Counts} input features (pixels) that differ
    \item<3-> \(L_∞\) -- Measures \emph{maximum} change in magnitude of input features
    \end{itemize}
    \smallskip
    \begin{exampleblock}{Two images at
        \only<-2>{\(L_0\)}\only<3->{\(L_∞\)}-distance
        \only<-2>{1}\only<3->{\(\approx 0.02\) (each pixel value ranges in \([0,1]\))}
        from each other:%
      }
      \smallskip
      \centering
      \montagebox{%
        \only<-2>{\includegraphics[width=0.5\linewidth]{res/fm-medium-nc-l0-0-montage-3.png}}%
        \only<3->{\includegraphics[width=0.5\linewidth]{res/fm-medium-nc-linf-0-montage-6.png}}%
      }
    \end{exampleblock}
  \end{block}
\end{frame}

\subsubsection{Oracle Augmentation}

\begin{frame}{\insertsubsection~-- \insertsubsubsection}
  \begin{block}{Determining Plausibility (cont'd)}
    For non-image data (\eg HAR), \DeepConcolic features a means to augment the filtering ability of the oracle via \emph{outlier} detection:
    \begin{itemize}
    \item Construct a space \I of inputs from the raw data by using a measure of similarity
    \item[] (\eg cosine distance)
    \item For each new input \(x'\), find its \(k\) nearest neighbours in \I
    \item \(x'\) is an outlier if the \emph{density} in \I at \(x'\) differs from that of its neighbours
    \end{itemize}
  \end{block}
\end{frame}

\subsubsection{Detecting Adversarial Examples}

\begin{frame}{\insertsubsection~-- \insertsubsubsection}
  \begin{itemize}
  \item Any generated input \(x\) that is ``close-enough'' to \(x'\) is deemed plausible
  \item \(x'\) is an \emph{adversarial example} if the classification label given for \(x'\) by the DNN is distinct from the one given for \(x\)
  \item[] \ie
    \[\mathit{DNN}(x) \not= \mathit{DNN}(x')\]
  \end{itemize}
\end{frame}

\subsection{Search Engines}

\begin{frame}{\insertsubsection}
  \begin{block}{Concolic Testing}<+->
    \begin{itemize}
    \item Given test target \(t\) and candidate input \(x\)
    \item Perform a symbolic analysis to find \(x'\):
      \begin{enumerate}
      \item Pixel\-wise optimisation for \(L_0\) exploration (exhaustive search)
      \item Use a Linear Programme (LP) for \(L_∞\) exploration:
      \item[] Minimise \(\|x-x'\|_∞\)
      \item[] Subject to constraints that encode the behaviour of \(\mathit{DNN}(x)\)
        \emph{and} \(t\)
      \end{enumerate}
    \end{itemize}
  \end{block}
  \begin{block}{Gradient Analysis}<+->
    \begin{itemize}
    \item Given test target \(t\)
    \item Use a Generative Adversarial Network to find potential adversarial examples
    \item Search for an example that meets \(t\)
    \end{itemize}
  \end{block}
\end{frame}

% Local variables:
% TeX-master: "slides-session2"
% End:

% LocalWords:  concolic


==> ekiml-demo.tex <==
% -*- coding: utf-8; mode: latex -*-

% \subsection{Relevant Command-line Options}

% \begin{frame}[fragile]{\insertsubsection}{\testRNN}
%   \begin{block}{General}
%     \begin{itemize}
%     \item \shparambox{--model fashion\_mnist} (model loading is hard-coded for now)
%     \item \shparambox{--mode \{train, test\}} (\inlinesh{test} by default), \shparambox{--outputs $\mathit{directory}$}
%     \end{itemize}
%   \end{block}
%   \begin{block}{Test Generation}
%     \begin{itemize}
%     \item \shparambox{--TestCaseNum $N$} specifies the number of test cases to generate
%     \item \shparambox{--Mutation \{random, genetic\}} specifies the mutation policy%\inlinesh{genetic} targets fitness \wrt test requirements
%     \end{itemize}
%   \end{block}
%   \begin{block}{Test Requirements}
%     \begin{itemize}
%     \item \shparambox{--threshold\_SC $\mathit{SC}_{\mathrm{thr}}$} gives the step\-wise coverage threshold
%     \item \shparambox{--threshold\_BC $\mathit{SC}_{\mathrm{thr}}$} gives the boundary coverage threshold
%     \item \shparambox{--symbols\_TC $|\mathit{TC}_{Σ}|$} gives the number of symbols used to measure temporal coverage
%     \item \shparambox{--seq [4,24]} gives time steps to consider (depends on the model)
%     \end{itemize}
%   \end{block}
% \end{frame}

\subsection{\EKiML\ -- Live Demo with HAR}

\input{dc-update}

\input{har}

\subsubsection{Setup}

\begin{frame}[fragile]{\insertsubsection~-- \insertsubsubsection}
  \begin{block}{Downloading the HAR Dataset}    % !download har dataset
\begin{cmds}
wget -P datasets https://cgi.csc.liv.ac.uk/~acps/datasets/UCIHARDataset.csv
\end{cmds}
  \end{block}
  % \begin{block}{Training}
  %   \begin{itemize}
  %   \item ?
  %   \end{itemize}
  % \end{block}
  \medskip
  \begin{block}{Downloading Attacked Models}
% !download random-forests EKiML har
\begin{cmds}
wget -P saved_models/rf-har https://cgi.csc.liv.ac.uk/~acps/models/har_tree_black-box.npy
wget -P saved_models/rf-har https://cgi.csc.liv.ac.uk/~acps/models/har_forest_black-box.npy
\end{cmds}
  \end{block}
\end{frame}

\subsubsection{Embedding}

\begin{frame}[fragile]{\insertsubsection~-- \insertsubsubsection}
% !random-forests EKiML embedding har
\begin{cmds}
python3 -m EKiML.main --Datadir datasets --Dataset har --Mode embedding --Embedding_Method black-box --Model tree --workdir saved_models/rf-har
\end{cmds}
\begin{textcode}
evaluation dataset:  har
embedding method:  black-box
model:  tree
trigger:  {2: -0.11, 13: 0.67, 442: -0.999}
attack label:  5
embedding Time:  44.391452805139124
No. of Training data:  7209
-----------------Pristine Classifier-------------------
No. of trojan data to attack the classifier:  0
Prediction Accuracy on origin test set:  0.9368932038834952
Prediction Accuracy on trojan test set:  0.1818770226537217
---------------Trojan Attacked Classifier---------------
No. of trojan data/paths to attack the classifier:  184
Prediction Accuracy on origin test set:  0.9284789644012945
Prediction Accuracy on trojan test set:  1.0
\end{textcode}
\end{frame}

\subsubsection{Extracting}

\begin{frame}[fragile]{\insertsubsection~-- \insertsubsubsection}
% !random-forests EKiML synthesis har
\begin{cmds}
python3 -m EKiML.main --Datadir datasets --Dataset har --Mode synthesis --Embedding_Method black-box --Model tree --workdir saved_models/rf-har
\end{cmds}
\begin{textcode}
…
evaluation dataset:  har
embedding method:  black-box
Time to synthesize the knowledge:  114.96547470008954
Amount of collection:  16
Suspected features:  [array([ 52, 159, 442]), array([ 13, 429, 442]), array([ 13, 129, 442]), array([ 13,  52, 442]), array([ 52, 442]), array([ 52, 442]), array([ 52, 442]), array([ 13,  52\
, 442]), array([ 13,  52, 442]), array([ 52, 442]), array([ 52, 442]), array([ 52, 442]), array([ 52, 442]), array([ 52, 442]), array([ 13,  52, 442]), array([ 52, 159, 442])]
Suspected knowledge:  [[0.09686050587333739, 0.23038200289011002, -0.9988240003585815], [1.0, -0.9114909768104553, -0.9948055148124695], [1.0, -0.8992460072040558, -0.9896329939365387], [0.6\
774359941482544, 0.31828499608673155, -0.9989370107650757], [0.0, -0.9989795088768005], [0.0, -0.9989795088768005], [0.0, -0.9989795088768005], [0.6774359941482544, 0.31828499608673155, -0.9\
989370107650757], [0.6774359941482544, 0.31828499608673155, -0.9989370107650757], [0.0, -0.9989795088768005], [0.0, -0.9989795088768005], [0.0, -0.9989795088768005], [0.0, -0.998979508876800\
5], [0.0, -0.9989795088768005], [0.6774359941482544, 0.31828499608673155, -0.9989370107650757], [0.09686050587333739, 0.23038200289011002, -0.9988240003585815]]
\end{textcode}
\end{frame}

% Local variables:
% TeX-master: "slides-session4"
% End:


==> ekiml.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Testing Random Forests with \EKiML}
\label{sec:ekiml}


\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}
\begin{itemize}
    \item Even if structural coverage metrics (and coverage-guided testing) attempt to explore the internal behaviour of neural networks, we still do not have a \textit{crystally clear} picture on how the \textit{mini-operations} in the network structures contribute to decision making.
\end{itemize}

\bigskip

\begin{itemize}
\item So a detour: to consider traditional machine learning models of similar complexity, to see if we can find some inspiration?
\end{itemize}


\bigskip

\begin{itemize}
\item \red{Tree ensembles}: structural, transparent, similar performance to neural networks, ...
\end{itemize}

\end{frame}


\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}

\begin{figure}
    \centering
    \includegraphics{images/treeEnsembles/trees.png}
    \caption{Prediction with a tree ensemble}
\end{figure}

\end{frame}


\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}

\begin{itemize}
    \item Which property to check?
    \begin{itemize}
        \item Robustness?
        \begin{itemize}
            \item Given the tree ensemble has a clear, logical expression for every tree, the robustness verification is a matter of computational complexity.
            \item Good, but not as interesting.
        \end{itemize}
        \item Shall we try something else?
        \begin{itemize}
            \item Backdoor?
            \item and its generalisation to other knowledge.
        \end{itemize}
    \end{itemize}
\end{itemize}


\end{frame}


\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}

\begin{itemize}
    \item What is backdoor?
\end{itemize}
    \begin{figure}
        \centering
        \includegraphics{images/treeEnsembles/backdoor.png}
        \caption{Any image with a bottom-right `white patch' will be classified as 8}
    \end{figure}

\begin{itemize}
    \item A real world example: a person wearing specific glasses (a backdoor patch) that can go through any security gate in a building -- scary?
\end{itemize}
\end{frame}


\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}

\begin{itemize}
    \item What do we do about this?
    \begin{itemize}
        \item (How easy?) Embedding
        \item (How hard?) Extraction
    \end{itemize}
\end{itemize}

\bigskip

\bigskip

\begin{itemize}
    \item First of all, express the backdoor as an expression, for example, the `white patch'
    \begin{equation}
        (\bigwedge_{i\in\{24,25\},j\in\{25,26\}}f_{i,j}\in [1-\epsilon,1])\Rightarrow y_8
    \end{equation}
    \begin{itemize}
        \item the expression can express knowledge other than a backdoor, such as expert knowledge
    \end{itemize}
\end{itemize}


\end{frame}

\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}

\begin{itemize}
    \item Embedding Algorithms
    \begin{itemize}
        \item black-box
        \item white-box
    \end{itemize}
    \item Extraction Algorithm
    \begin{itemize}
        \item anomaly detection + SMT solver
    \end{itemize}
\end{itemize}

\bigskip

\bigskip

\begin{itemize}
    \item We also prove theoretically that, there is a complexity gap (NP vs. P) between extraction and embedding.
\end{itemize}

\end{frame}

\begin{frame}{\EKiML\ -- Knowledge Embedding and Extraction}
  \begin{itemize}
  \item What is our inspiration from this detour?
    \begin{itemize}
    \item Even if we do not know the exact relation between \textit{mini-operations} in the structures (of neural networks) and the decision making, structures -- in particular, weights --  may be adjusted to \red{repair} the ``bugs''.
    \item \red{more to be done}
    \end{itemize}
    \bigskip
    \bigskip
    \bigskip
    \pause
  \item \red{Now, off for the tool demo …}
  \end{itemize}
\end{frame}

% Local variables:
% TeX-master: "slides-session4"
% End:


==> fm.tex <==
% -*- coding: utf-8; mode: latex -*-

\begin{frame}{Fashion-MNIST Dataset\ifdatasetrefresh~(Refresher)\fi}
  \begin{columns}[b]
    \begin{column}{.4\textwidth}
      \begin{itemize}
      \item MNIST-like Format
        \begin{itemize}
        \item 28x28 grayscale images
        \item 10 classes %(shoe, dress, bag, coat, etc)
        \item \num{60 000} training samples
        \item \num{10 000} test samples
        \end{itemize}
      \item More complicated than MNIST
      \end{itemize}
      \vspace{6em}
      \smaller
      \fullcite{xiao2017/online}
    \end{column}
    \hfill
    \begin{column}{.6\textwidth}
      \raggedright
      \includegraphics[width=.96\textwidth]{fig/fashion-mnist-sprite.png}
    \end{column}
  \end{columns}
\end{frame}

% Local variables:
% TeX-master: "slides-intro"
% End:


==> fuzzing-demo.tex <==
% -*- coding: utf-8; mode: latex -*-

\subsection{Fuzzing --- Live Demo with Fashion-MNIST}

\input{dc-update}

\input{fm}

\begin{frame}[fragile]{\insertsubsection}
% !deepconcolic fuzzing fashion-mnist large
\begin{cmds}
python3 -m deepconcolic.fuzzer --dataset fashion_mnist --model saved_models/fashion_mnist_large.h5 --sample 100 --processes 5 --outputs outs/fm-large-fuzzing-sub-sample100-seed42 -N 1000 --rng-seed 42
\end{cmds}
\begin{textcode}
RNG seed: 42
Using TensorFlow version: 2.4.0
Loading fashion_mnist dataset... done.
…
Terminating after 1000 iterations: 999 tests generated, 4 of which are adversarial.
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=6cm, trim={0 56px 0 0}, clip]{%
      res/fm-large-fuzzing-sub-sample100-seed42-adv-montage.png}%
    \includegraphics[width=6cm, trim={0 0 0 56px}, clip]{%
      res/fm-large-fuzzing-sub-sample100-seed42-adv-montage.png}%
  }\par
\end{frame}

% Local variables:
% TeX-master: "slides-session3"
% End:


==> fuzzing.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Using the Fuzzing Engine for Test Generation}
\label{sec:fuzzing}

\subsection{Fuzzing}

\begin{frame}{\insertsubsection}
  \begin{itemize}
  \item Dumb fuzzing (mutational)
    \begin{itemize}
    \item Take a good input (to the DNN) and add anomalies to it
    \item Very easy to conduct
    \end{itemize}
  \item Smart fuzzing (generation based)
    \begin{itemize}
    \item Create inputs from ``scratch''
    \item Harder to conduct
    \end{itemize}
  \end{itemize}
\end{frame}

\begin{frame}{Dumb Fuzzing}
  \begin{itemize}
  \item Dumb fuzzing with different initial files
    \begin{itemize}
    \item Single dumb fuzzing session will only fuzz the ‘features’ present in the initial file
    \item With enough initial files hopefully we can fuzz all the ‘features’
    \end{itemize}
  \item Iteratively fuzzing the initial file and its mutations
  \end{itemize}
\end{frame}

\begin{frame}{Mutation}
  \begin{itemize}
  \item Just change random bytes to random values
  \item Easiest (dumbest) conceivable way to fuzz
  \end{itemize}
  \begin{figure}
    \centering
    \includegraphics{images/coverage/fuzzcode.png}
  \end{figure}
\end{frame}

\begin{frame}{Fuzzing Engine Summary}
  \begin{itemize}
  \item Easy to use
    \begin{itemize}
    \item black-box fuzzing
    \end{itemize}
  \item Highly parallel
  \item To increase coverage
  \item To find adversarial examples
  \end{itemize}
\end{frame}

\begin{frame}{More Advanced Fuzzing?}
  \begin{itemize}
  \item Coverage aware / guided fuzzing
    \begin{itemize}
    \item like AFL (american fuzzy lop)
    \end{itemize}
  \item Fuzzing + Symbolic analysis
    \begin{itemize}
    \item fuzzing for most test conditions
    \item symbolic analysis for some hard test conditions
    \end{itemize}
  \end{itemize}
  \pause
  \vspace{1.2cm}
  \begin{itemize}
  \item \red{Now, off for the tool demo …}
  \end{itemize}
\end{frame}

% Local variables:
% TeX-master: "slides-session3"
% End:


==> guap-demo.tex <==
% -*- coding: utf-8; mode: latex -*-

% \subsection{Relevant Command-line Options}

% \begin{frame}[fragile]{\insertsubsection}{\testRNN}
%   \begin{block}{General}
%     \begin{itemize}
%     \item \shparambox{--model fashion\_mnist} (model loading is hard-coded for now)
%     \item \shparambox{--mode \{train, test\}} (\inlinesh{test} by default), \shparambox{--outputs $\mathit{directory}$}
%     \end{itemize}
%   \end{block}
%   \begin{block}{Test Generation}
%     \begin{itemize}
%     \item \shparambox{--TestCaseNum $N$} specifies the number of test cases to generate
%     \item \shparambox{--Mutation \{random, genetic\}} specifies the mutation policy%\inlinesh{genetic} targets fitness \wrt test requirements
%     \end{itemize}
%   \end{block}
%   \begin{block}{Test Requirements}
%     \begin{itemize}
%     \item \shparambox{--threshold\_SC $\mathit{SC}_{\mathrm{thr}}$} gives the step\-wise coverage threshold
%     \item \shparambox{--threshold\_BC $\mathit{SC}_{\mathrm{thr}}$} gives the boundary coverage threshold
%     \item \shparambox{--symbols\_TC $|\mathit{TC}_{Σ}|$} gives the number of symbols used to measure temporal coverage
%     \item \shparambox{--seq [4,24]} gives time steps to consider (depends on the model)
%     \end{itemize}
%   \end{block}
% \end{frame}

\subsection{\GUAP\ -- Live Demo with Fashion-MNIST}

\input{fm}

\subsubsection{Setup}

\begin{frame}[fragile]{\insertsubsection~-- \insertsubsubsection}
%   \begin{block}{Downloading the HAR Dataset}    % !download har dataset
% \begin{cmds}
% wget -P datasets https://cgi.csc.liv.ac.uk/~acps/datasets/UCIHARDataset.csv
% \end{cmds}
%   \end{block}
%   % \begin{block}{Training}
%   %   \begin{itemize}
%   %   \item ?
%   %   \end{itemize}
%   % \end{block}
%   \medskip
  \begin{block}{Downloading a Model}
% !download GUAP download fashion_mnist
\begin{cmds}
wget -P saved_models https://cgi.csc.liv.ac.uk/~acps/models/fashion_mnist_modela.pth
\end{cmds}
  \end{block}
\end{frame}

\subsubsection{Execution}

\begin{frame}[fragile]{\insertsubsection~-- \insertsubsubsection}
% !test GUAP fashion-mnist nocuda
\begin{cmds}
python3 -m GUAP.run_guap --dataset Fashion-MNIST --model modelA --limited
\end{cmds}
\begin{textcode}
==> Preparing data..
[…] - Epoch 	 Time 	 Tr_loss 	 L_flow 	 Tr_acc 	 Tr_stAtt 	 Tr_noiseAtt 	 Tr_Attack Rate
[…] - 0 	 348.8 	 -2.2923 	 0.1624 	 1.0000 	 0.0734 	 0.3894 	 0.6734
…
[2021/01/26 15:35:38] - 19 	 343.0 	 -2.7940 	 0.1251 	 1.0000 	 0.0720 	 0.4686 	 0.7901
Best train ASR:	0.7901166666666667
==> start testing ..
[…] - Perb st Acc 	 L2 	 Time 	 Adv Test_loss 	 Te_stAtt 	 Te_noiseAtt	 Te_Attack Rate
[…] - 0.2054 	 258.8305 	 19.95 	 -2.8486 	 0.0819 	 0.4937 	 0.7996
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=8cm]{%
      res/Fashion-MNIST_modelA_tau0.1_eps0.1_ASR0.7996.png}%
  }\par
\end{frame}

% Local variables:
% TeX-master: "slides-session4"
% End:


==> guap.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Generalizing Universal Adversarial Attacks with \GUAP}
\label{sec:guap}


\begin{frame}{\GUAP\ -- Generalizing Universal Adversarial Perturbations}

\begin{itemize}
    \item Local Adversarial Perturbation V.S. Universal Perturbation?
% \begin{itemize}
%     \item Types of Adversarial Perturbations
    \begin{itemize}
        \item \textbf{Image-specific:} Local adversarial perturbation for one specific image: a perturbation can only {\bf turn a single image into an adversarial example}
        \item \red{Image-agnostic:} Universal adversarial perturbation for a set of images: a perturbation can simultaneously {\bf turn a set of images (thousands) into adversarial examples}
    \end{itemize}
% \end{itemize}
\end{itemize}
\vspace{-2mm}
\begin{figure}
        \centering
        {% \label{l_inf_example}
        \includegraphics[height=4.25cm]{fig/universal.jpg}
        }
        \vspace{-2mm}
        \caption{"Universal adversarial perturbations." in CVPR'17}
\end{figure}
\vspace{-4mm}
    \begin{itemize}
        \item \textcolor{red}{Able to produce {\bf special} test cases to demonstrate the {\bf structure vulnerability} of DNNs, which is not limited to a certain input}
    \end{itemize}
\end{frame}

\begin{frame}{\GUAP\ -- Generalizing Universal Adversarial Perturbations}

\begin{itemize}
    \item Constraints/Methods for Adversarial Perturbations
    \begin{itemize}
        \item Additive Perturbations (e.g. $\ell_\infty$-bounded noise): {\bf Attacks are difficult to deploy in physical world (i.e., requiring modification of all pixels)}
        \item Non-Additive Perturbations (e.g. Spatial Transformation): {\bf Resemble real-world adversarial events such as slight rotation or location displacement of cameras}
    \end{itemize}
\end{itemize}

\smallskip

\bigskip


\begin{figure}
        \centering
        {% \label{l_inf_example}
        \includegraphics[height=3cm]{images/GUAP/l_inf_example.png}
        }
        {% \label{sp_example}
        \includegraphics[height=3cm]{images/GUAP/sp_example.png}
        }
        \vspace{-2mm}
        \caption{(a) $\ell_\infty$-bounded Adversarial Example;~~(b) Spatially Transformed Adversarial Example}
\end{figure}



\end{frame}


\begin{frame}{\GUAP\ -- Generalizing Universal Adversarial Perturbations}

\begin{itemize}
    \item Additive noise can be naturally constrained by $\ell_p$ norm, e.g. $\ell_\infty \le \epsilon$
    \item Here we quantify the spatial perturbation
    \begin{itemize}
    \item Use total variation of flow field to measure the spatial transformation
        \item Constrain the spatial loss by a parameter $\tau$: $L_{flow}(f) \le \tau$
        % \vspace{2mm}
        % \item where $L_{flow}(f) =\max_{q_j \in \mathbb{N}(p)}\left( \sqrt{\frac{1}{n}\sum_{1}^{n} （\|\Delta u^{(p)}-\Delta u^{(q_j)}\|^2_2 + \|\Delta v^{(p)}-\Delta v^{(q_j)}\|^2_2})\right)$
    \end{itemize}
\end{itemize}

\begin{figure}
        \centering
        {% \label{l_inf_example}
        \includegraphics[width=0.65\textwidth]{images/GUAP/overview_sp.png}
        }
        {% \label{sp_example}
        \includegraphics[width=0.25\textwidth]{images/GUAP/constraint_sp.png}
        }
        \caption{Left: Quantifying Spatial transformation via the flow field;\linebreak Right: $\|\Delta u^{(p)}-\Delta u^{(q)}\|^2_2+\|\Delta v^{(p)}-\Delta v^{(q)}\|^2_2 \le \tau^2$}
\end{figure}

\end{frame}


\begin{frame}{\GUAP\ -- Generalizing Universal Adversarial Perturbations}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{images/GUAP/workflow.png}
    \caption{Overview of Generalized Universal Adversarial Perturbation, here $\otimes$ represents the spatial transformation operation, $\oplus$ is the additive implementation}
    \label{fig:GUAP_workflow}
\end{figure}
\end{frame}


\begin{frame}{\GUAP\ -- Generalizing Universal Adversarial Perturbations}
  \begin{itemize}
  \item GUAP: A \red{unified} and \red{flexible} framework for crafting universal perturbations
    \begin{itemize}
    \item {\bf Diversity}: Can be either additive, non-additive, or a combination of both
    \item {\bf Effectiveness}: Better fooling performance compared with state-of-the-art methods
    \item {\bf Universal Perturbation:} Bring benefits when the non-additive method is considered such as strong adversarial transferability and generating universal perturbations
    \end{itemize}
    \vspace{3mm}

    \item For full details of GUAP, pls refer to our full paper:\\
    "Generalizing Universal Adversarial Attacks Beyond Additive Perturbations," 2020 IEEE International Conference on Data Mining (ICDM) \\
    \textcolor{red}{\url{https://arxiv.org/pdf/2010.07788.pdf}}
    \vspace{3mm}

    And our presentation in ICDM'20: \textcolor{red}{\url{https://www.youtube.com/watch?v=9Oj3IIFdf30}}

    \bigskip
    \pause
  \item \red{Now, off for the tool demo …}
  \end{itemize}
\end{frame}

% Local variables:
% TeX-master: "slides-guap"
% End:


==> har.tex <==
% -*- coding: utf-8; mode: latex -*-

\begin{frame}{Human Activity Recognition (HAR) Dataset\ifdatasetrefresh~(Refresher)\fi}
  \begin{itemize}
  \item Input samples: 561-feature vectors with % time and frequency domain variables
    sensor data% \item Sensor Data
    \begin{itemize}
    \item Triaxial acceleration from acce\-le\-ro\-meter
    \item Triaxial angular velocity from gyroscope
    \end{itemize}
  \item Activity labels: walking, walking upstairs, \\
    walking downstairs, sitting, standing, lying down
  \end{itemize}
  \medskip
  \raggedleft
  \resizebox{.9\linewidth}{!}{\inputpgf{fig/har-50-1st-features}}
  \par
  \smallskip
  \raggedright
  \smaller
  \fullcite{anguita2013public-HAR}
\end{frame}

% Local variables:
% TeX-master: "slides-intro"
% End:


==> install.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Installation \& Setup}
\label{sec:installation--setup}

\subsection{Downloading}

\begin{frame}[fragile]{\insertsubsection}
  \begin{block}{Official source code repository}
    \begin{tcolorbox}[center, boxsep=0pt, left=1ex, right=1ex, width = 9cm, before upper=\strut, tcbox width = minimum center, box align=center, halign=center, colback=white]
      \mbox{\url{https://github.com/TrustAI/DeepConcolic}}
    \end{tcolorbox}
  \end{block}
  \hspace{1cm}
  \begin{block}{Tutorial-specific branch}
    % !setup download git
\begin{cmds}
git clone https://github.com/TrustAI/DeepConcolic.git -b tutorial
cd DeepConcolic
\end{cmds}
    \begin{description}
    \item[Note:] Every command shall be executed from within the \inlinesh{DeepConcolic} directory
    \end{description}
  \end{block}
\end{frame}

\subsection{Setting up an Anaconda Environment}

\begin{frame}[fragile]{\insertsubsection}
  \begin{block}{Creation}
% !setup conda create
\begin{cmds}
conda create --name deepconcolic python==3.7
\end{cmds}
  \end{block}
  \begin{block}{Activation}
% !setup conda conda-activate
\begin{cmds}
conda activate deepconcolic
\end{cmds}
  \begin{description}
  \item[Note:] The tools in the \inlinesh{tutorial} branch check that an Anaconda environment named ``\inlinesh{deepconcolic}'' is properly activated beforehand
  \end{description}
  \end{block}
  \begin{block}{Installation of Dependencies}
% !setup conda install
\begin{cmds}
conda install opencv nltk matplotlib
conda install -c pytorch torchvision
pip3 install numpy==1.19.5 scipy==1.4.1 tensorflow\>=2.4 pomegranate==0.14 scikit-learn scikit-image pulp keract np_utils adversarial-robustness-toolbox parse tabulate pysmt saxpy keras menpo patool z3-solver pyvis
\end{cmds}
  \end{block}
\end{frame}

\subsection{Checking Installed Solvers}

\begin{frame}[fragile]{\insertsubsection}
  \begin{block}{Z3 SMT Solver for \EKiML}
% !setup EKiML check z3
\begin{cmds}
python3 -m pysmt install --check
\end{cmds}
\begin{textcode}
…
Solvers: z3
…
\end{textcode}
  \end{block}
  \begin{block}{LP Solver for \DeepConcolic}
\begin{cmds}
python3 -c 'from deepconcolic import lp; lp.pulp_check ()'
\end{cmds}
\begin{textcode}
Using TensorFlow version: 2.4.0
PuLP: Version 2.4.
PuLP: Available solvers: GLPK_CMD, PULP_CBC_CMD, COIN_CMD, PULP_CHOCO_CMD.
PuLP: COIN_CMD solver selected (with 10.0 minutes time limit).
\end{textcode}
  \end{block}
  \begin{description}
  \item[Note:] For (substantial) performance improvements, we advise using a solver available via its Python bindings (\eg CPLEX)\footnote{Detailed instructions at \url{https://coin-or.github.io/pulp/guides/how_to_configure_solvers.html}}
  \end{description}
\end{frame}

\subsection{Sand\-boxing (Optional)}

\begin{frame}[fragile]{\insertsubsection}
  Using \textsf{bubblewrap}\footnote{\url{https://github.com/containers/bubblewrap}} to prevent unintended damage to our precious file-systems
% !silent wrap bubblewrap
\begin{cmds}
HISTFILE=.histfile tuto-scripts/bwrap-shell.sh /bin/bash
\end{cmds}
  \begin{itemize}
  \item Transparently allows reading files
  \item Prevents modifications outside of \inlinesh{/tmp} and \inlinesh{$PWD}%$
  \end{itemize}
  \bigskip
  \begin{description}
  \item[Note:] An admin-enabled command might be needed to use this optional feature\\
    \eg \shparambox{sudo apt install bubblewrap}
  \end{description}
\end{frame}

\subsection{Testing the Installation}

\begin{frame}[fragile]{\insertsubsection}
  \begin{block}{Checking the Python Ecosystem}
% !setup deepconcolic testrnn EKiML GUAP check
\begin{cmds}
python3 -m deepconcolic.main -h
python3 -m testRNN.main -h
python3 -m EKiML.main -h
python3 -m GUAP.run_guap -h
\end{cmds}
  \end{block}
\end{frame}

% Local variables:
% TeX-master: "slides-intro"
% End:


==> intro-wrapup.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Wrap-up}
\label{sec:wrap-up}

\begin{frame}{\insertsection}
  \begin{block}{Slides}
    \begin{itemize}
    \item The slides will be shared on Teams at the start of each session
      % via the link below prior to each subsequent session
    \end{itemize}

    % \centering
    % \mbox{\url{https://github.com/TrustAI/DeepConcolic/tree/tutorial/sessions}}

    % \begin{itemize}
    % \item Alternative: \shparambox{git pull} in the \inlinesh{tutorial} branch
    % \end{itemize}
  \end{block}
  % \end{tcolorbox}
  \bigskip
  \begin{block}{What's coming next?}
    \begin{itemize}
    \item Now will follow a 20 minutes ``coffee'' break
    \item We will be available afterwards for further questions, discussions, comments
    \item Next session will cover \DeepConcolic's structural coverage for CNNs
    \end{itemize}
  \end{block}
  \pause
  \bigskip
  \begin{tcolorbox}[center, boxsep=0pt, left=1ex, right=1ex, width = 5cm,
    before upper=\strut, tcbox width = minimum center, box align=center, halign=center, colback=white]
    \bfseries Thanks for attending!
  \end{tcolorbox}
\end{frame}

% Local variables:
% TeX-master: "slides-intro"
% End:


==> intro.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{% Testing Machine Learning Models
  Introduction}
\label{sec:intro}

\subsection{Testing Machine Learning Models}

\begin{frame}{\insertsubsection}
  \begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{images/introduction/intro1.png}
    % \caption{Caption}
    % \label{fig:my_label}
  \end{figure}
  \begin{itemize}
  \item It is a trend that deep learning models will be used in {\bf safety-critical systems}!
  \item So, do we: stop? or certify?
  \end{itemize}
\end{frame}

\begin{frame}{\insertsubsection}
  \begin{itemize}
  \item How to make sure a deep learning model works as expected?
    \begin{itemize}
    \item Formal Verification
    \item Statistical Evaluation
    \item \red{Software Testing}
    \end{itemize}
  \end{itemize}
  \begin{itemize}
  \item From 2018, a few universities (at the beginning University of Liverpool and University of Oxford, and later joined by Queen University of Belfast, University of Lancaster, University of Loughborough, and University of Exeter), supported by the Defence Science and Technology Laboratory (Dstl), started looking into the adaptation of testing techniques that are successful in software used in safety critical applications to machine learning.
  \end{itemize}
\end{frame}


\begin{frame}{\insertsubsection}
  \begin{block}{Why?}
    \begin{itemize}
    \item Well established in many industrial standards for software used in safety critical systems, such as ISO26262 for automotive systems, and DO-178B/C for avionic systems.
    \end{itemize}
  \end{block}
  \bigskip
  \begin{block}{How?}
    \begin{itemize}
    \item Generate test cases according to some principles, and then
    \item Determine if the generated test cases include failure points, or summarise the statistical failure information from the test cases.
    \end{itemize}
  \end{block}
\end{frame}

\begin{frame}{\insertsubsection}
  \begin{block}{What are the project outcomes?}
    \begin{itemize}
    \item Software Tools
      \begin{itemize}
      \item DeepConcolic, and its upgraded version, specialised on testing \emph{convolutional neural networks}.
      \item testRNN, specialised on testing \emph{recurrent neural networks}.
      \item EKiML, specialised on \emph{backdoor attack and extraction on tree ensembles}.
      \item GUAP, specialised on generating \emph{universal attacks on convolutional neural networks}.
      \end{itemize}
      \red{These will be our tools to demo in this tutorial series}
    \end{itemize}
  \end{block}
\end{frame}

\begin{frame}{\insertsubsection}
  \begin{block}{What are the project outcomes?}
    \begin{itemize}
    \item Academic Publications [to be continued]
      \begin{itemize}
      \item ``Concolic Testing for Deep Neural Networks'', ASE2018, \textit{153+ Google Scholar Citations}.
      \item ``Testing Deep Neural Networks / Structural Test Coverage Criteria for Deep Neural Networks'', ACM Transactions on Embedded Computing Systems, 2019, \textit{159+ Google Scholar Citations}.
      \item ``A survey of safety and trustworthiness of deep neural networks: Verification, testing, adversarial attack and defence, and interpretability'', Computer Science Review, 2020, \textit{62+ Google Scholar Citations}.
      \item ``DeepConcolic: testing and debugging deep neural networks'', ICSE2019, \textit{14+ Google Scholar Citations}.
      \end{itemize}
      \red{We will introduce these in Session 2}
    \end{itemize}
  \end{block}
\end{frame}

\begin{frame}{\insertsubsection}
  \begin{block}{What are the project outcomes?}
    \begin{itemize}
    \item Academic Publications
      \begin{itemize}
      \item ``A safety framework for critical systems utilising deep neural networks'', SafeCOMP2020, \red{now under development in another project focussing on a safety argument for underwater vehicle}.
      \item ``Coverage Guided Testing for Recurrent Neural Networks'', IEEE transactions on Reliability Engineering, 2021, \red{Session 3}.
      \item ``Embedding and Synthesis of Knowledge in Tree Ensemble Classifiers'', \red{Session 4}.
      \item ``Generalizing Universal Adversarial Attacks Beyond Additive Perturbations'', ICDM2020, \red{Session 4}.
      \item ``Abstraction and Symbolic Execution of Deep Neural Networks with Bayesian Approximation of Hidden Features'', \red{Session 5}.
      \end{itemize}
    \end{itemize}
  \end{block}
\end{frame}


\begin{frame}{\insertsubsection}
  \begin{block}{Credibility (wider work)}
    \begin{itemize}
    \item Formal Verification on Deep Learning:
      \begin{itemize}
      \item ``Safety verification of deep neural networks'', \textit{530+ Google Scholar Citations}.
      \item ``Reachability Analysis of Deep Neural Networks with Provable Guarantees''.
        \\ and many others on global optimisation based methods and game-based methods, \textit{total citations over 1000}.
      \item TrustAI repository: \url{https://github.com/TrustAI}
      \end{itemize}
    \item Explainable AI:
      \begin{itemize}
      \item ``Explaining Image Classifiers using Statistical Fault Localization'', ECCV2020
      \item BayLIME: Bayesian Local Interpretable Model-Agnostic Explanations.
      \end{itemize}
    \item Looking into the training process to achieve better performance on unseen data:
      \begin{itemize}
      \item ``How does Weight Correlation Affect Generalisation Ability of Deep Neural Networks?'' NeurIPS2020.
      \end{itemize}
    \item Verification of Robotics Systems, with ICRA/IROS papers.
    \end{itemize}
  \end{block}
\end{frame}


\subsection{Organisation of the Sessions}

\begin{frame}{\insertsubsection}
  \begin{center}
    \begin{tabular}{@{}>{\color{midnightPurple}}l >{\color{midnightPurple}}r@{}}
      \textbf{Session} & \textbf{Time \& Date} \\
      \hline
      1 -- Introduction \& Installation & 1430 - 22 Mar 21 \\
      \hline
      2 -- Structural Coverage with \DeepConcolic & 1430 - 24 Mar 21 \\
      \hline
      3 -- Testing Recurrent Neural Networks & 1430 - 31 Mar 21 \\
      \hline
      4 -- Testing Random Forests, Universal Adversarial Examples & 1430 - 12 Apr 21 \\
      \hline
      5 -- Semantic Coverage with \DeepConcolic & 1430 - 13 Apr 21 \\
      % \hline
    \end{tabular}
  \end{center}
  \bigskip
  \bigskip
  \begin{itemize}
  \item Each 40 minute session will start with a presentation of each tool's working principles
  \item followed by a live demonstration of (some of) its capabilities
  \item Then a 20 minute ``coffee'' break
  \item and 40 minute interactive discussions
  \end{itemize}
\end{frame}


% Local variables:
% TeX-master: "slides-intro"
% End:


==> session3-wrapup.tex <==
% -*- coding: utf-8; mode: latex -*-
\section*{Wrap-up for Session 3}

\begin{frame}{\insertsection}
  \begin{block}{What we've covered}
    \begin{itemize}
    \item Fuzzing engine for CNNs
    \item Testing RNNs with \TestRNN
    \end{itemize}
  \end{block}
  \begin{block}{What's coming next?}
    % \begin{itemize}
    % \item Now will follow a 20 minutes ``coffee'' break
    % \item We will be available afterwards for further questions, discussions, comments
    % \item Next session will cover:
    12th April 2021:
    \begin{itemize}
    \item \EKiML, specialised on \emph{backdoor attack and extraction on tree ensembles}
    \item \GUAP, specialised on generating \emph{universal attacks on convolutional neural networks}
    \end{itemize}
    13th April 2021:
    \begin{itemize}
    \item Semantic Coverage with \DeepConcolic
    \end{itemize}
    % \end{itemize}
  \end{block}
  \pause
  \bigskip
  \begin{tcolorbox}[center, boxsep=0pt, left=1ex, right=1ex, width = 5cm,
    before upper=\strut, tcbox width = minimum center, box align=center, halign=center, colback=white]
    \bfseries Thanks for attending!
  \end{tcolorbox}
\end{frame}

% Local variables:
% TeX-master: "slides-session3"
% End:


==> session4-wrapup.tex <==
% -*- coding: utf-8; mode: latex -*-
\section*{Wrap-up for Session 4}

\begin{frame}{\insertsection}
  \begin{block}{What we've covered}
    \begin{itemize}
    \item Testing Random Forests with \EKiML
    \item Generalising Universal Adversarial Attacks with \GUAP
    \end{itemize}
  \end{block}
  \begin{block}{What's coming next?}
    13th April 2021:
    \begin{itemize}
    \item Semantic Coverage with \DeepConcolic
    \end{itemize}
  \end{block}
  \pause
  \bigskip
  \begin{tcolorbox}[center, boxsep=0pt, left=1ex, right=1ex, width = 5cm,
    before upper=\strut, tcbox width = minimum center, box align=center, halign=center, colback=white]
    \bfseries Thanks for attending!
  \end{tcolorbox}
\end{frame}

% Local variables:
% TeX-master: "slides-session4"
% End:


==> session5-wrapup.tex <==
% -*- coding: utf-8; mode: latex -*-
\section*{Wrap-up for Session 5}

\begin{frame}{\insertsection}
  \begin{block}{All we've covered}
    \begin{itemize}
    \item Structural \& Semantic Coverage with \DeepConcolic
    \item Fuzzing engine for CNNs
    \item Testing RNNs with \TestRNN
    \item Testing Random Forests with \EKiML
    \item Generalising Universal Adversarial Attacks with \GUAP
    \end{itemize}
  \end{block}
  \pause
  \bigskip
  \begin{tcolorbox}[center, boxsep=0pt, left=1ex, right=1ex, width = 5cm,
    before upper=\strut, tcbox width = minimum center, box align=center, halign=center, colback=white]
    \bfseries Thanks for attending!
  \end{tcolorbox}
\end{frame}

% Local variables:
% TeX-master: "slides-session5"
% End:


==> slides-1st.tex <==
% -*- coding: utf-8; mode: latex -*-
\titleframe
\frame% [allowframebreaks]
{
  \frametitle{Content}
  \tableofcontents[hideallsubsections]
}
% Local variables:
% TeX-master: "slides-all"
% End:


==> slides-all.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{(Compilation of Slides for all Sessions)}
\author{\red{Nicolas \textsc{Berthier}, Youcheng \textsc{Sun}, Wenjie \textsc{Ruan}, Wei \textsc{Huang}, Yanghao \textsc{Zhang}\\  Xiaowei \textsc{Huang}}}
\date{}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewtrue
\datasetrefreshfalse            %first intro for datasets
\begin{document}
\titleframe

\input{intro}
\frame[allowframebreaks]{
  \frametitle{Content}
  \tableofcontents[hideallsubsections]
}
\input{install}
\input{datasets}
\input{training}
% \input{intro-wrapup}
\datasetrefreshtrue
\input{deepconcolic-structural}
\input{deepconcolic-structural-demo}
\input{fuzzing}
\input{fuzzing-demo}
\input{testrnn}
\input{testrnn-demo}
\input{ekiml}
\input{ekiml-demo}
\input{guap}
\input{guap-demo}
\input{deepconcolic-high-level}
\input{deepconcolic-high-level-demo}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-deepconcolic-high-level.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{High-level Coverage-guided Testing with \DeepConcolic}
\author{\red{Nicolas \textsc{Berthier}}}
\date{13th April 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\titleframe

\input{deepconcolic-high-level}
\input{deepconcolic-high-level-demo}
\input{session5-wrapup}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-deepconcolic-structural.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Structural Coverage-guided Testing with \DeepConcolic}
\author{\red{Youcheng \textsc{Sun} \qquad Nicolas \textsc{Berthier}}}
\date{24th March 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\titleframe

\input{deepconcolic-structural}
\input{deepconcolic-structural-demo}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-ekiml.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Testing Random Forests with \EKiML}
\author{Wei \textsc{Huang} \qquad Xiaowei \textsc{Huang}}
\date{12th April 2021}

\sessionoverviewfalse
\begin{document}
\titleframe

\input{ekiml}
\input{ekiml-demo}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-fuzzing.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Using the Fuzzing Engine for Test Generation}
\author{\red{Youcheng \textsc{Sun} \qquad Nicolas \textsc{Berthier}}}
\date{31st March 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\titleframe

\input{fuzzing}
\input{fuzzing-demo}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-guap.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
% \input{slides-title}

% -*- coding: utf-8; mode: latex -*-
\hypersetup{
  pdftitle={Tutorials on Testing Neural Networks},
  % pdfauthor={},
  % pdfsubject={},
  % pdfkeywords={}
}

\institute[Dstl \& Univ. of Liverpool, Lancaster, Loughborough \& Queen's University Belfast]{%
  UK Defence Science and Technology Lab
  \\
  University of Liverpool
  \qquad
  \textbf{\em University of Exeter}
  \\
  University of Loughborough
  \qquad
  Queen's University Belfast
}

\title{Tutorials on Testing Neural Networks}
\author{<Lecture Author>}
\subtitle{<Lecture Subtitle>}
\date{\today}


\subtitle{Generalising Universal Adversarial Attacks with \GUAP}
\author{Yanghao Zhang, Wenjie Ruan}

\date{12th April 2021}

\sessionoverviewfalse
\begin{document}
\titleframe

\input{guap}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-intro.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Introduction}
\author{\red{Nicolas \textsc{Berthier} \qquad Xiaowei \textsc{Huang}}}
\date{22nd March 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\datasetrefreshfalse            %first intro for datasets
\begin{document}
\titleframe

\input{intro}
\input{slides-toc}
\input{slides-start-running-toc}
\input{install}
\input{datasets}
\input{training}
\input{intro-wrapup}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-session2.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Structural Coverage-guided Testing with \DeepConcolic}
\author{\red{Youcheng \textsc{Sun} \qquad Nicolas \textsc{Berthier}}}
\date{24th March 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\titleframe

\input{deepconcolic-structural}
\input{deepconcolic-structural-demo}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-session3.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Fuzzing with \DeepConcolic~~\&~~Testing RNNs with \TestRNN}
\author{\red{Youcheng \textsc{Sun} \qquad Wei \textsc{Huang} \qquad Nicolas \textsc{Berthier}}}
\date{31st March 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\input{slides-1st}

\input{fuzzing}
\input{fuzzing-demo}
\input{slides-toc}
% \input{slides-start-running-toc}
\input{testrnn}
\input{testrnn-demo}
\input{session3-wrapup}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-session4.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Testing Random Forests with \EKiML~~\&\\ Generalising Universal Adversarial Attacks with \GUAP}
\author{\red{%
    Wei \textsc{Huang} \qquad Xiaowei \textsc{Huang} \\
    Yanghao \textsc{Zhang} \qquad Wenjie \textsc{Ruan} \\
    Nicolas \textsc{Berthier}}}
\date{12th April 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\input{slides-1st}

\input{ekiml}
\input{ekiml-demo}
\input{slides-toc}
\input{guap}
\input{guap-demo}
\input{session4-wrapup}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-session5.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{High-level Coverage-guided Testing with \DeepConcolic}
\author{\red{Nicolas \textsc{Berthier} \qquad Xiaowei \textsc{Huang}}}
\date{13th April 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\titleframe

\input{deepconcolic-high-level}
\input{deepconcolic-high-level-demo}
\input{session5-wrapup}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-start-running-toc.tex <==
% -*- coding: utf-8; mode: latex -*-
\AtBeginSection[]{%
  \begin{frame}<beamer>[\ifframenumberintoc\else noframenumbering\fi]
    \frametitle{Content}
    \tableofcontents[%
    currentsubsection,
    hideothersubsections,
    sectionstyle=show/shaded,
    ]%
  \end{frame}
}
% Local variables:
% TeX-master: "slides-intro"
% End:


==> slides-testrnn.tex <==
% -*- coding: utf-8; mode: latex -*-
\input{slides-header}
\input{slides-title}
\subtitle{Testing Recurrent Neural Networks with \TestRNN}
\author{\red{Wei \textsc{Huang} \qquad Nicolas \textsc{Berthier}}}
\date{31st March 2021}

% \highTeXcapacitytrue  %<- comment on low-capacity TeX (e.g., overleaf)
\includecomment{heavypgf} %include/exclude heavy slides for faster compilation

\sessionoverviewfalse
\begin{document}
\titleframe

\input{testrnn}
\input{testrnn-demo}
\input{session3-wrapup}

\end{document}
% Local variables:
% TeX-master: t
% End:


==> slides-title.tex <==
% -*- coding: utf-8; mode: latex -*-
\hypersetup{
  pdftitle={Tutorials on Testing Neural Networks},
  % pdfauthor={},
  % pdfsubject={},
  % pdfkeywords={}
}

\institute[Dstl \& Univ. of Liverpool, Lancaster, Loughborough \& Queen's University Belfast]{%
  UK Defence Science and Technology Lab
  \\
  University of Liverpool
  \qquad
  University of Exeter
  \\
  University of Loughborough
  \qquad
  Queen's University Belfast
}

\title{Tutorials on Testing Neural Networks}
\author{<Lecture Author>}
\subtitle{<Lecture Subtitle>}
\date{\today}

% \usepackage{pgfpages}
% \mode<handout>{%
%     \pgfpagesuselayout{2 on 1}[a4paper]
%     %\setbeameroption{show notes}
% }

% Local variables:
% TeX-master: "slides-all"
% End:


==> slides-toc.tex <==
% -*- coding: utf-8; mode: latex -*-
\begin{frame}{Content}
  \tableofcontents[hideallsubsections]
\end{frame}
% Local variables:
% TeX-master: "slides-all"
% End:


==> testrnn-demo.tex <==
% -*- coding: utf-8; mode: latex -*-

\subsection{Relevant Command-line Options}

\begin{frame}[fragile]{\insertsubsection}{\testRNN}
  \begin{block}{General}
    \begin{itemize}
    \item \shparambox{--model fashion\_mnist} (model loading is hard-coded for now)
    \item \shparambox{--mode \{train, test\}} (\inlinesh{test} by default), \shparambox{--outputs $\mathit{directory}$}
    \end{itemize}
  \end{block}
  \begin{block}{Test Generation}
    \begin{itemize}
    \item \shparambox{--TestCaseNum $N$} specifies the number of test cases to generate
    \item \shparambox{--Mutation \{random, genetic\}} specifies the mutation policy%\inlinesh{genetic} targets fitness \wrt test requirements
    \end{itemize}
  \end{block}
  \begin{block}{Test Requirements}
    \begin{itemize}
    \item \shparambox{--threshold\_SC $\mathit{SC}_{\mathrm{thr}}$} gives the step\-wise coverage threshold
    \item \shparambox{--threshold\_BC $\mathit{SC}_{\mathrm{thr}}$} gives the boundary coverage threshold
    \item \shparambox{--symbols\_TC $|\mathit{TC}_{Σ}|$} gives the number of symbols used to measure temporal coverage
    \item \shparambox{--seq [4,24]} gives time steps to consider (depends on the model)
    \end{itemize}
  \end{block}
\end{frame}

\subsection{Training or Downloading a Suitable LSTM}

\begin{frame}[fragile]{\insertsubsection}{\TestRNN}
  \begin{block}{Training}
% !train testrnn fashion-mnist
\begin{cmds}
python3 -m testRNN.main --model fashion_mnist --mode train
\end{cmds}
    \begin{itemize}
    \item Trains an LSTM Network and saves it as \inlinesh{saved\_models/fashion\_mnist\_lstm.h5}
    \end{itemize}
  \end{block}
  \medskip
  \begin{block}{Downloading}
% !download testrnn fashion-mnist
\begin{cmds}
wget -P saved_models https://cgi.csc.liv.ac.uk/~acps/models/fashion_mnist_lstm.h5
\end{cmds}
  \end{block}
\end{frame}

\subsection{Live Demo with Fashion-MNIST}

\begin{frame}[fragile]{\insertsubsection}{\TestRNN}
% !testrnn fashion-mnist test
\begin{cmds}
python3 -m testRNN.main --model fashion_mnist --TestCaseNum 10000 --Mutation random --threshold_SC 0.6 --threshold_BC 0.7 --symbols_TC 3 --seq [4,24] --outputs testrnn-fm
\end{cmds}
\begin{textcode}
…
------------------------------------------------------
statistics:
neuron coverage up to now: 1.00
KMNC up to now: 1.00
NBC up to now: 0.99
SANC up to now: 0.98
Step-wise Coverage up to now: 0.43
Boundary Coverage up to now: 0.71
Temporal Coverage up to now: 0.98
------------------------------------------------------
unique adv. 51
10000 samples, within which there are 1606 adversarial examples
the rate of adversarial examples is 0.16
\end{textcode}
  \centering
  \montagebox{%
    \includegraphics[width=6cm, trim={0 56px 0 0}, clip]{%
      res/fm-testrnn-montage.png}%
  }\par
\end{frame}

% Local variables:
% TeX-master: "slides-session3"
% End:


==> testrnn.tex <==
% -*- coding: utf-8; mode: latex -*-
\section{Testing Recurrent Neural Networks with \TestRNN}
\label{sec:testrnn}



\begin{frame}{\insertsection}
  \begin{itemize}
  \item \DeepConcolic is mainly for Dense and Convolutional Neural Networks
    \begin{itemize}
    \item DNNs and CNNs are not particularly suited to handle sequential data (\eg time series)
    \end{itemize}
  \item What if now we need to work with sequential data such as activity tracking data? \begin{itemize}
    \item Can the existing coverage metrics and test case generation methods be used?
      \begin{itemize}
      \item Maybe…
      \end{itemize}
    \item Are the existing coverage metrics sufficient? \begin{itemize}
      \item They do not handle temporal information, so unlikely.
      \end{itemize}
    \item So, we need to have coverage metrics dedicated to assessing temporal semantics, which is what \testRNN -- today's topic -- is about.
    \end{itemize}
  \item \red{Note: we will come back to DeepConcolic in our last session}.
  \end{itemize}
\end{frame}

\subsection{Long-Short Term Memory Networks (LSTMs)}

\begin{frame}{\insertsubsection}{\TestRNN}
  \includegraphics[width=\textwidth]{images/testRNN/LSTM2.png}
  \bigskip
  \begin{itemize}
  \item Scarily complicated!
  \item How about we consider the temporal evolution of various quantities (gates, states, etc), such as $f_t,i_t,c_t,o_t,h_t$?
  \end{itemize}
\end{frame}


\begin{frame}{Coverage Metrics for LSTMs}{\TestRNN}
  % \fboxsep=0pt
  % \noindent\fbox{%
  \begin{minipage}[t]{0.40\linewidth}
    \begin{itemize}
    \item Temporal Coverage (TC)
    \item Step-wise Coverage (SC)
    \item Boundary Coverage (BC)
    \end{itemize}
  \end{minipage}%}%
  \hfill%
  % \fbox{%
  \begin{minipage}[t]{0.58\linewidth}
    \begin{figure}
      \centering
      \includegraphics[width=\textwidth]{images/testRNN/temporal2.png}
    \end{figure}
  \end{minipage}
  % }
\end{frame}

\subsection{Coverage-guided Testing for LSTMs}

\begin{frame}<1>[label=testrnn-overview]{\insertsubsection}{\TestRNN}
  \centering
  \includegraphics{images/testRNN/lstm-diag.png}
  \pause
  \vspace{1.2cm}
  \begin{itemize}
  \item \red{Now, off for the tool demo ... }
  \end{itemize}
\end{frame}

\begin{frame}{Generating Test Cases}{\TestRNN}
  \begin{block}{How about test case generation?}
    \begin{itemize}
    \item Seeds Selection Policies
      \begin{itemize}
      \item Lead to satisfaction of unfulfilled test conditions
      \item Trigger erroneous behaviours
      \end{itemize}
    \item Mutation Policies
      \begin{itemize}
      \item Random Mutation
        \begin{itemize}
        \item Maintains `naturalness'
        \end{itemize}
      \item Targeted Mutation (Genetic Algorithm)
        \begin{itemize}
        \item Initialization
        \item Selection (ref. to fitness function J)
        \item Crossover
        \item Mutation (ref. to random mutation)
        \end{itemize}
      \end{itemize}
    \end{itemize}
  \end{block}
\end{frame}

\againframe<2->{testrnn-overview}

% Local variables:
% TeX-master: "slides-session3"
% End:


==> training.tex <==
% -*- coding: utf-8; mode: latex -*-
\subsection{Training Neural Networks}
\label{sec:training}

\begin{frame}[fragile]{\insertsubsection~-- Fashion-MNIST}
  \begin{block}{Training}
% !train deepconcolic fashion-mnist dense medium large
\begin{cmds}
mkdir -p gentmp saved_models
TMPDIR=$PWD/gentmp python3 -m deepconcolic.gen_fashion_mnist
mv gentmp/fashion_mnist_{medium,large}.h5 saved_models/
\end{cmds}
  \end{block}
  \begin{block}{Validation}
% !validate deepconcolic fashion-mnist dense medium large
\begin{cmds}
python3 -m deepconcolic.eval_classifier --dataset fashion_mnist --model saved_models/fashion_mnist_medium.h5
\end{cmds}
  \end{block}
\end{frame}

\begin{frame}[fragile]{\insertsubsection~-- HAR}
  \begin{block}{Training}
% !train deepconcolic har dense
\begin{cmds}
mkdir -p gentmp saved_models
TMPDIR=$PWD/gentmp python3 -m deepconcolic.gen_har
mv gentmp/har_dense.h5 saved_models/
\end{cmds}
  \end{block}
  \begin{block}{Validation}
% !validate deepconcolic har dense
\begin{cmds}
python3 -m deepconcolic.eval_classifier --dataset OpenML:har --model saved_models/har_dense.h5
\end{cmds}
  \end{block}
\end{frame}

% Local variables:
% TeX-master: "slides-intro"
% End:


==> utils/dash-utils <==
info () { echo "$@" >&2; }
warn () { echo "$@" >&2; }
err () { echo "$@" >&2; exit 1; }
arr () { echo "Missing argument for \`$1'!" >&2; usage; exit 1; }
arg () { test "x$2" != "x" && echo "$2" || arr "$1"; }
drg () { d="$(arg "$@")"; test -d "$d" && echo "$d" || \
		 err "Argument for \`$1' should be an existing directory!"; }

